Ad Auctions for LLMs via Retrieval Augmented Generation

In the field of computational advertising, the integration of ads into the outputs of large language models (LLMs) presents an opportunity to support these services without compromising content integrity. This paper introduces novel auction mechanisms for ad allocation and pricing within the textual outputs of LLMs, leveraging retrieval-augmented generation (RAG). We propose a segment auction where an ad is probabilistically retrieved for each discourse segment (paragraph, section, or entire output) according to its bid and relevance, following the RAG framework, and priced according to competing bids. We show that our auction maximizes logarithmic social welfare, a new notion of welfare that balances allocation efficiency and fairness, and we characterize the associated incentive-compatible pricing rule. These results are extended to multi-ad allocation per segment. An empirical evaluation validates the feasibility and effectiveness of our approach over several ad auction scenarios, and exhibits inherent tradeoffs in metrics as we allow the LLM more flexibility to allocate ads.

==> further.tex <==
\section{Appendix}


\begin{definition}[Proportional fairness]
    An allocation $\x \in \Delta_n$ is proportionally fair with weights $\w$ if for any other allocation $\y \in \Delta_n$, it satisfies
    \begin{align*}
        \sum_{i \in [n]} w_i\frac{y_i - x_i}{x_i} \le 0
    \end{align*}
\end{definition}

\begin{theorem}[\cite{kelly1998rate}]
    The allocation $\x(\q,\b) \in \Delta_n$ maximizes  $\LogEff$ if and only if it is proportionally fair with weights $(q_iv_i)_{i \in [n]}$.
\end{theorem}
\sscomment{Also mention CEEI, and say by [Arrow and Intriligator 1982, Volume 2, Chapter 14, MNW coincides CEEI.}


\section{Temp - we may need it}


\subsection{Parameterized mechanism}
We here introduce a generalized mechanism that interpolates the EPIC and FAIR mechanisms obtained above.
Consider the following allocation rule.
\begin{align*}
    x_i(\q, \b) = \frac{(q_ib_i + f(q_i))^{\eta}}{\sum_{j \in \cA} (q_jb_j + f(q_j))^{\eta}}
\end{align*}
\sscomment{But this does not have explicit antiderivative formula.}


\sscomment{TODO: This subsection needs to be fixed. Figure out what is this maximizing. Also, fix the equations since we changed $b_i$ to be $\tb_i$. Probably better to put this in the appendix.}
In this settings, we consider a softmax allocation which is controlled by an external parameter $\eta$.
In fact, as $\eta \to \infty$, this softmax allocation acts as a hardmax allocation function while at $\eta \to 0$ it mimics a uniform allocation function with any preferences over advertisers.
To be more formal, allocation function is defined as follows:

\begin{align}
    x_a(\q,\b) = \frac{e^{\eta q_a b_a}}{\sum_{i \in \cA} e^{\eta q_i b_i}}.\label{eq:alloc-temp}
\end{align}

Applying~\eqref{eq:myerson-pay} on ~\eqref{eq:alloc-temp}, our payment rule will be
\begin{align*}
    p_a(q_a, b_a, \q_{-a}, \b_{-a}) = \int_{0}^{b_a} z \cdot \frac{d}{dz}\left(\frac{e^{\eta q_a b_a}}{\sum_{i \in \cA} e^{\eta q_i b_i}}\right) dz \, .
\end{align*}
Write $w = \sum_{a \neq i, a \in \cA} e^{\eta q_i b_i}$.
We obtain the integral as follows 
\begin{align}
    p_a(q_a, b_a, \q_{-a}, \b_{-a}) 
    &= \int_{0}^{b_a} z \cdot \frac{d}{dz}\left(\frac{e^{\eta q_a z}}{w + e^{\eta q_a z}}\right) dz \nonumber
    \\
    &= \int_{0}^{b_a} z \cdot \left(\frac{w \cdot \eta q_a e^{\eta q_a z}}{(w + e^{\eta q_a z})^2}\right) dz \nonumber
    \\
    &= \int_{0}^{b_a} \frac{w \cdot \eta q_a e^{\eta q_a z} z}{(w + e^{\eta q_a z})^2} dz  \nonumber
    \\
    &= - \frac{w z}{e^{\eta q_a z} + w} + z - \frac{1}{\eta q_a} \ln{\left(e^{\eta q_z z} + w\right)} \Big|_0^{b_a} \nonumber
    \\
    &=
    b_a - \frac{b_a w}{e^{\eta q_a b_a} + w} + \frac{1}{\eta q_a} \ln{\left(\frac{1+w}{e^{\eta q_a b_a} + w}\right)} \, .
\end{align}

In the above formula, $\eta$ determines how sensitive the mechanism is to values of $q_a b_a$. 
\sscomment{TODO: Provide a picture, and say that it is first convex and then concave after a point.}

\begin{theorem}
    Consider RAG-based LLM advertising auction with base probability $\q$ and bids $\b$.
    The following mechanism $\Mec$ is DSIC:
    \begin{align}
        \Mec = (\x, \p) = \left( \frac{e^{\eta q_a b_a}}{\sum_{i \in \cA} e^{\eta q_i b_i}},
        b_a - \frac{b_a w}{e^{\eta q_a b_a} + w} + \frac{1}{\eta q_a} \ln{\left(\frac{1+w}{e^{\eta q_a b_a} + w}\right)}
        \right) \, .
    \end{align}
\end{theorem}


% \paragraph{Allocation function}
% If all the advertisers write the same bids for their ads, we can allocate each ad $a$ with probability $\CPru{\eta}{a}{x}$ as in the original RAG-sequence model.
% \sscomment{Issue: allocation vector needs to sum up to $1$. Originally $\sum_{a}\CPru{\eta}{a}{x}$ is not necessarily $1$. Any other candidates that sum up to $1$? Or we can simply normalize. It might be the case that $y$ should be also accounted to represent the relevance.}

% Suppose that each ad $a$ is equipped with a bid $b_a \in \R_{\ge 0}$.
% What will be the expected revenue of advertising $a$?
% It is simply $b_a$.
% What is the potential loss of advertising $a$?
% It is opportunity cost of transmitting a possibly undesirable ad.
% How much each ad $a$ is desirable originally?
% $\CPru{\eta}{a}{x}$.
% Then how should we change the allocation vector?
% Write $q_a = \CPru{\eta}{a}{x}$.
% Then a simple version of adjusted allocation probability is
% \begin{align}
%     x_a = x_a (q_a, b_a; q_{-a},b_{-a}) = \frac{q_a b_a}{\sum_{i \in \cA} q_i b_i}.
% \end{align}

% Given the allocation vector $x = (x_a)_{a \in \cA}$, the following Myerson's lemma states that the payment function can be uniquely computed.
% \begin{lemma}[\cite{myerson1981optimal}]
    
% \end{lemma}


% A nuanced approach might be to parameterize
% \begin{align}
%     x_a = \CPru{\eta}{a}{x} \cdot \frac{e^{\theta \cdot b_a}}{\sum_{a \in \cA} e^{\theta \cdot b_a}/ |\cA|} \, .
% \end{align}



\sscomment{BELOW IS OLD}
---------------------------------------------

We first introduce several notations. 

Given $A = \{i_1,\ldots, i_k\} \in \cA_k$, we write $b_A = \{b_{i_1},\ldots, b_{i_k}\}$ and $a_A = \{a_{i_1},\ldots, a_{i_k}\}$.

\subsection{Output selection}
Suppose we want to advertise $k$ ads at once given a query $x$.
Note that the choice of $k$ can be endogenous to the mechanism but for simplicity, we here assume that $k$ is an exogenous parameter for now.
Assuming that we have selected the set of ads $A = \{i_1,i_2,\ldots, i_k\}$, we mainly consider the following equation from a variant of RAG-sequence model to determine the eventual output
\begin{align}
    \CPr{y}{x} = \CPru{\eta}{A}{x} \CPru{\theta}{y}{x,A} \, .\label{eq:comb}
\end{align}
Equation~\eqref{eq:comb} exactly replaces the single ad $a_1$ in~\eqref{eq:single} with the tuple $A$.
Correspondingly, the final output $y$ will be selected by $\argmax_y \CPr{y}{x}$ similar to the~\cite{lewis2020retrieval}.
We often write $y_A$ to denote the corresponding output given selected $A$.


% We first consider two approaches to determine how the eventual output $y$ can be determined assuming that a set of ads $\{a_1,a_2,\ldots, a_k\}$ to advertise at once is determined.

% \sscomment{For marginalized selection: it seems not reasonable to charge both, since it is just conditioning a single ad.}
% \begin{definition}
%     We define two types of mechanisms as follows.
%     \begin{enumerate}
%         \item In the \emph{marginalized selection}, we compute the following probability.
%         \begin{align*}
%             \CPr{y}{x} = \sum_{i \in [k]}\CPru{\eta}{a_i}{x} \CPru{\theta}{y}{x,a_i} \, ,
%         \end{align*}
%         and select $\argmax_y \CPr{y}{x}$.
%         \item On the other hand, in the \emph{combinatorial selection}, we compute
%         \begin{align*}
%             \CPr{y}{x} = \CPru{\eta}{a_1,a_2,\ldots, a_k}{x} \CPru{\theta}{y}{x,a_1,a_2,\ldots, a_k} \, ,
%         \end{align*}
%         and select $\argmax_y \CPr{y}{x}$.
%     \end{enumerate} 
%     \sscomment{Another way is to consider RAG-token}
% \end{definition}
% \sscomment{Sebastien's question: normalizing?}

% Pros of the marginalized selection is that the mechanism, especially the allocation function can be more efficiently implemented.
% However, the output $y$ will be more likely to advertise a single ad rather than advertising multiple ads at once.

% The advantage of the combinatorial selection is that it is more likely to be advertising multiple ad at once since we give the multiple ads as documents to generate a single output $y$.
% The cons is that it might be more inefficient as discussed shortly.

\subsection{Warm-up: naive BA mechanism}
To select the $k$ out of every possible ads $\cA$, we start with a naive approach as a warm up.
This approach will give us insights what should further be considered as a feature of the multiple allocation mechanism distinguished from the single allocation mechanism.
For ease of exposition, we first introduce ideal mechanisms regardless of the computational complexity, and then present computationally tractable mechanisms to approximate the ideal ones, in a similar vein to~\cite{hartline2009simple}.

% \paragraph{Marginalized selection}
% First consider deterministic mechanism.
% For example if $k = 2$, we compute maximum $b_iq_i$ and second-highest $b_jq_j$, and then run VCG auction, which is to charge them the price that makes the quantity at least third highest $b_k q_k$.

% What about randomized mechanism?
% Sampling two ads:
% \begin{align}
%     x_a(\q,\b) = \frac{q_a b_a}{\sum_{i \in \cA} q_i b_i}.\label{eq:alloc}
% \end{align}


% In words, in the aggregated distribution model, we aggregate the probability distribution for multiple ads, and sample the output.
% On the other hand in the Pairwise RAG model, more complicated extension to group the set of documents simultaneously in a combinatorial manner.


% \paragraph{Warm up - naive approach}
% \sscomment{As mechanism is independent from output selection, we may use simpler quantity like $p(a_i|x) + p(a_j | x)$.}
Similar to the single allocation setting, our mechanism, in particular the allocation function, can be obtained as follows.
\begin{definition}[Naive MA mechanism]\label{def:naive-ma}
    A naive MA mechanism $\Mec = (\x, \p)$ is fully specified as follows.
    \begin{enumerate}
        \item Collect bids $\b = (b_1,\ldots, b_n) \in \R^n$.
        \item Compute baseline probability vector $q_A = \CPru{\eta}{A}{x}$ according to~\eqref{eq:comb} for every $A \in \cA_k$.
        \item {\bf Allocation rule}: select $A^* = \argmax_{A \in \cA_k} v_A$ where $v_A = \sum_{a \in A}b_a \cdot \CPru{\eta}{A}{x}$, \ie
        \begin{align}
            x_i(\q_k, \b) = \begin{cases}
                            1 \mbox{ if $i \in A^*$} \\ 
                            0 \mbox{ otherwise}
                        \end{cases} \label{eq:naive-ma-alloc}
        \end{align}
        where we write $\q_k = (q_A)_{A \in \cA_k}$.
        \item {\bf Payment rule}: compute payment $\p(\q_k, \b) \in \R^n$ from Myerson's lemma~\ref{lem:myerson}.
    \end{enumerate}
\end{definition}


One can easily see that the proposed allocation rule is monotone over $\b$.
\begin{proposition}
    The allocation rule given by Definition~\ref{def:naive-ma} is monotone over $\b$.    
\end{proposition}
\begin{proof}
    \sscomment{fix notation}
    For arbitrary $i \in [n]$, fix $b_{-i}$ and consider $b_i \ge b'_i$.
    If $i \in A^*$ with bid $b'_i$, then it follows that
    \begin{align*}
        \sum_{a \in A}b_a \cdot \CPru{\eta}{A}{x} \ge \sum_{a \in A}b'_a \cdot \CPru{\eta}{A}{x},
    \end{align*}
    implying that $i \in A^*$ with bid $b_i$.
\end{proof}

To more elaborate on the explicit payment formula, similar to the second price auction, fix an index $i \in [n]$.
According the Myerson's lemma, when increasing $a_i$'s bid $z$, the integrand becomes exactly $1$ only if $i$ starts to be included in the selected set $A^*$.
Precisely, it computes the lowest possible $z$ such that there exists $B \in \cA_{k-1}$ such that the following holds:
\begin{align}
    (z + \sum_{j \in B}b_j) \CPru{\eta}{B \cup \{z\}}{x} \ge \max_{C \in \cA_{k}: i \notin C} \sum_{a \in C}b_a \CPru{\eta}{C}{x} \, , \label{eq:naive-ma-pay}
\end{align}
and charge advertiser $a_i$ the price $z$ if it is selected in $A^*$.

This approach, however, requires the following fundamental assumption in the advertiser's valuation.
\begin{assumption}\label{as:naive-ma}
    The advertiser's $a_i$'s true value for being included in any winner package $A \in \cA_k$ is $b_i$.
\end{assumption}

Thus, we obtain the following theorem.

\begin{theorem}
    Consider RAG auction with multiple allocation with base probability $(\q_A)_{A \in \cA_k}$ and bids $\b$.
    The naive MA mechanism with allocation rule given by~\eqref{eq:naive-ma-alloc} and payment rule given by~\eqref{eq:naive-ma-pay} is DSIC under the Assumption~\ref{as:naive-ma}.
\end{theorem}

\sscomment{question: it is not completely clear whether the resulting mechanism would be truthful. Bidder only writes $b_1$, and we manually define adjusted bid. Still, given the allocation rule, we define the payment according to the Myerson, it may be truthful. For example, suppose that we multiply $100$ at the both hand sides of~\eqref{eq:naive-ma-alloc}, then payment would become $100$ times the bid.}





% First consider deterministic mechanism.
% For example if $k = 2$, we compute
% \begin{align*}
%     (b_i + b_j)\CPru{\eta}{a_i,a_j}{x},
% \end{align*}
% and pick the maximal one, \eg $a_1$ and $a_2$.
% For $a_1$, we charge minimum $z$ such that
% \begin{align}
%     (z + b_2)\CPru{\eta}{a_1,a_2}{x} \ge \max_{i,j \neq 1}(b_i + b_j)\CPru{\eta}{a_i, a_j}{x} \, , \label{eq:comb-naive}
% \end{align}
% and similarly for $a_2$.
% According to the 


% \sscomment{Further compute the payment function here.}



\begin{discussion}
    Importantly, however, Assumption~\ref{as:naive-ma} restricts the platform to always run $k$-allocation mechanism regardless of the query and number of available or relevant ads.
    In addition, each advertiser is enforced to write a single dimensional bid regardless of the package $A$ that its ad will be advertised together.
    This way, 
    
    would the payment function above make sense from advertiser's perspective?
    Essentially, if multiple ads are simultaneously advertised in a single output, then the impact of marketing decreases compared to the SA mechanism. 
    Yet, the advertisers are charged based on their written bids $\b$ which do not account for the MA mechanism.
    Thus, the proposed naive mechanism may significantly dissatisfy the advertiser's utility, possibly inducing the low participation of the advertisers.    
\end{discussion}

As per the discussion above, to attract more advertisers, the platform needs to offer a better protocol to efficiently communicate with the advertiser to reflect their needs with respect to the output of the mechanism.

A simple approach to overcome such a challenge is to ask each advertiser to write every bid $b$ for every possible tuple $A \in 2^{\cA}$, or for $A \in \cA_k$.
This way, however, obviously bothers the advertisers too much as they need to write a menu of exponential size for 
Moreover, since the set of available ads are significantly dynamic in practice, thus this approach seems to be highly impractical.


% should use different bid other than $\b$ for MA mechanism in case the advertisers are asked to write $\b$ for SA mechanism.
% We consider the following two approaches to this end: (i) explicitly ask the advertisers to write multi dimensional bids and (ii) maintain the single-dimensional bid, but adjust the bid $\b$ based on some reasonable measures on the output.
% We begin by explaining the second approach and turns our attention to the first one.\footnote{\sscomment{Or one may compute the minimal $\rho$ such that
% \begin{align*}
%     \rho (b_1 + b_2)\CPru{\eta}{a_1,a_2}{x} 
%     \ge 
%     \max_{i,j \neq 1}(b_i + b_j)\CPru{\eta}{a_i, a_j}{x}  \, ,
% \end{align*}
% and determine the total bid $\rho(b_1 + b_2)$ and then define a payment sharing mechanism separately.}}



\subsection{Bid adjustment mechanism}
To overcome the challenge exhibited in the naive MA mechanism above, we suggest a nuanced but efficient protocol to collect the bid.
We first formally introduce the bid adjust mechanism as follows.
\begin{definition}[Bid adjustment mechanism]
    Consider a $k$-MA setting.
    A bid adjustment (BA) mechanism $\Mec = (\x, \p, F)$ is fully specified as follows.
    \begin{enumerate}
        \item Announce bid adjustment function $F:\R^k \times (\Theta^*)^{k+2} \mapsto \R^k$ such that $F(b_A, a_A, x, y_A) = \hat{b}_A$ given $A \in \cA_k$.\footnote{Note that the bid adjustment mechanism subsumes the naive MA mechanism by defining $F$ such that $F(b_A, a_A, x, y_A) = b_A$.}
        \item Collect bids $\b = (b_1,\ldots, b_n) \in \R^n$.
        \item Compute baseline probability vector $q_A = \CPru{\eta}{A}{x}$ according to~\eqref{eq:comb} for every $A \in \cA_k$.
        \item {\bf Allocation rule}: select $A^* = \argmax_{A \in \cA_k} v_A$ where $v_A = ||F(b_A, a_A, x, y_A)||_1 \cdot \CPru{\eta}{A}{x}$, \ie
        \begin{align}
            x_i(\q_k, \b) = \begin{cases}
                            1 \mbox{ if $i \in A^*$} \\ 
                            0 \mbox{ otherwise}
                        \end{cases}
        \end{align}
        where we write $\q_k = (q_A)_{A \in \cA_k}$.
        \item {\bf Payment rule}: compute payment $\p(\q_k, \b) \in \R^n$ from Myerson's lemma~\ref{lem:myerson}.
    \end{enumerate}
\end{definition}
\sscomment{n choose k call to relenvace oracle. (n choose k) times k computatin for allocation rule. Then for payment, we require n choose k times k, and then fix B, then find z.}

\paragraph{Similarity-based adjustment}
\sscomment{One subtle thing: $P(A | x)$ should not appear in the advertiser's utility. Probably in the naive setting, this can be viewed as allocative efficiency, etc?}
The key ingredient of bid adjustment mechanism is the bid adjustment function $F$.
We first propose a \emph{similarity-based} BA mechanism.
Essentially we use the probability $\CPr{a_i}{y_A, x}$ for $i \in A$ as an estimate of the similarity (relevance) of ad $a_i$ for the output $y_A$ given the query $x$.
Then, given a tuple $A \in \cA_k$ and a bid adjustment mechanism $\Mec = (\x, \p, F)$, we define $F$ as follows.
\begin{align}
    F(b_A, a_A, x, y_A) 
    = b_A 
    = \left( \CPr{a_{i_1}}{y_A} \cdot b_{i_1}, \ldots,  \CPr{a_{i_k}}{y_A} \cdot b_{i_k}  \right) \, ,\label{eq:ba-f}
\end{align}
where $a_{i_j}$'s bid is adjusted to be $\hat{b}_{i_j} = \CPr{a_{i_j}}{y_A} \cdot b_{i_j}$ for $j \in [k]$.\footnote{\sscomment{To avoid bias, multiple samples for $P(a_1 | y_A)$ and average? Take one output?}}

In fact, the foundation of our function above grounds on the following assumption.
\begin{assumption}
    The true valuation for $y_A$ for $a_{i}$ is $\CPr{a_i}{y_A}\cdot b_{i}$.\footnote{\sscomment{Mention that we can also have this one in the single allocation setting}}
\end{assumption}

\sscomment{Ideal mec: exponentially multi dimensional mechanism. Cannot change the ad but only bid. Define valuation in the beginning.}

\begin{discussion}
    We remark that computing $\CPr{a}{y_A}$ for some $A \in \cA_k$ and $i \in A$ essentially entails the marginalization over all possible $j \in [n]$.
    More precisely, using Bayes' rule we obtain
    \begin{align*}
        \CPr{a_i}{y_A,x} = \frac{\CPr{y_A}{a_i,x} \cdot \CPr{a_i}{x}}{\sum_{j \in [n]} \CPr{y_A}{a_j,x}} .
    \end{align*}
    Note in fact that if the ads are fairly distinguishable, the summation in the denominator might boil down to the summation over $\sum_{j \in A}$, which would decrease the computational complexity.
\end{discussion}



% Consider $k$-allocation setting.
% Among $\cA$, we should choose $k$ ads to advertise.

% Consider the tuple $A = a_1,\ldots, a_k$.
% First, $\CPr{a_1,a_2,\ldots, a_k}{x}$ is the selection probability.
% For the tuple $A$, there will be corresponding output $y_A$.
% Then, we can calculate the relevance $\CPr{a_1}{y_A}$, \ie the relevance between $a_1$ and $y_A$.
% Now we adjust our bid by computing
% \begin{align}
%     F(b_A, a_A, x, y_A) = \CPr{a_1}{y_A} \cdot b_1 + \ldots + \CPr{a_k}{y_A} \cdot b_k \, .
% \end{align}


Thus, as per~\eqref{eq:comb-general}, the final value for tuple $A$ is given by
\begin{align}
    v_A = \parans{\CPr{a_{i_1}}{y_A} \cdot b_{i_1} + \ldots + \CPr{a_{i_k}}{y_A} \cdot b_{i_k}} \cdot \CPr{a_1,a_2, \ldots, a_k}{x} \, . \label{eq:comb-adjust}
\end{align}
Thus, the allocation function is to select the tuple $A$ that maximizes the equation~\eqref{eq:comb-adjust}.\footnote{\sscomment{it also makes sense to consider parameterized one or threshold}}

\begin{proposition}
    The allocation rule defined from~\eqref{eq:comb-adjust} is monotone over $\b$.
\end{proposition}
\begin{proof}
    For arbitrary $i_1 \in [n]$, fix $(b_{i_2},b_{i_3},\ldots, b_{i_K})$ and consider $b_{i_1} \ge b'_{i_1}$.
    If $i \in A^*$ with bid $b'_i$, then it follows that
    \begin{align*}
        &\left( \CPr{a_{i_1}}{y_A} \cdot b_{i_1} + \ldots + \CPr{a_{i_k}}{y_A} \cdot b_{i_k} \right) \cdot \CPr{a_{i_1},a_{i_2}, \ldots, a_{i_k}}{x}
        \\
        &\ge
        \parans{\CPr{a_{i_1}}{y_A} \cdot b'_{i_1} + \ldots + \CPr{a_{i_k}}{y_A} \cdot b_{i_k}} \cdot \CPr{a_{i_1},a_{i_2}, \ldots, a_{i_k}}{x}
    \end{align*}
    implying that $i_1 \in A^*$ with bid $b_{i_1}$.
\end{proof}

According the Myerson's lemma, similar to the naive MA mechanism, the payment rule for ad $a_{i}$ is given by the lowest possible $z$ such that there exists $B \in \cA_{k-1}$ that the following holds:
\begin{align}
    F(b_{B \cup \{z\}}, a_{B \cup \{z\}}, x, y_{B \cup \{z\}}) \cdot \CPru{\eta}{B \cup \{z\}}{x} 
    \ge 
    \max_{C \in \cA_{k}: i \notin C} F(b_{C}, a_{C}, x, y_{C}) \CPru{\eta}{C}{x} \, , \label{eq:simil-ma-pay}
\end{align}
and charge advertiser $a_{i}$ the price $z \cdot \CPr{a_{i_1}}{y_A, x}$ if it is selected in $A^*$.\footnote{This is because we consider $\Pr{a_{i_1}}{y_A} \cdot z$ as the entire \emph{adjusted bid}. This would result in the same consequence if we use $z' + \sum_{j \in [k] \setminus \{1\}}\CPr{a_{i_j}}{y_A,x} \cdot b_{i_j}$ as the adjusted bid and select the lowest $z'$ in a similar manner.}

Thus, the following theorem follows.
\begin{theorem}
    Consider RAG auction with multiple allocation with base probability $(\q_A)_{A \in \cA_k}$ and bids $\b$.
    The BA mechanism with allocation rule given by~\eqref{eq:comb-adjust} and payment rule given by~\eqref{eq:simil-ma-pay} is DSIC.
\end{theorem}



\paragraph{Relative adjustment}
Suppose we are running the similarity-based BA mechanism with $k = 2$ and $n =3$.
Assume further that $A = \{a_1, a_2\}$ are selected to be advertised as per the mechanism above, given a query $x$ and corresponding output $y_A$.

Let us compare this to another case of when we were to run a single allocation mechanism and $a_1$ is selected.
Suppose that, in extreme and in hindsight, it turns out that $y_A$ under the MA mechanism happens to be very similar (or equivalent) to $y_{a_1}$ under the SA mechanism.
Then, a natural question arises: in hindsight, would we really need to adjust (lower) the bid $b_1$ under the MA mechanism for advertiser $1$?

Since the output themselves are exactly equivalent from $a_1$'s perspective, we don't actually need to lower the bid $b_1$ to offer a reasonable payment scheme to the advertiser.
How can we change our bid adjustment function $F(\cdot)$ to adapt to this case?
One approach would be to use the ratio between $\CPr{y_A}{a_1, x}$ and $\CPr{y_1}{a_1,x}$ to adjust the bid, formally defined as follows.

\begin{definition}[Relative adjustment]
    
\end{definition}



\begin{discussion}[Relative mechanism]
    How about comparing $\CPr{a_1}{y_1}$ and $\CPr{a_1}{y_A}$ and then adjust bid based on them? Basically so that if $y_1$ is very similar to $y_A$ we may not actually need to adjust the bid, since the advertisement effect might remain almost the same, which is pretty reasonable.
    Just considering $\CPr{a_1}{y_A}$ does not account for the relative effect like above.
    In case of two-allocation mechanism, if $y_{ij}$ is very similar to both $y_i$ and $y_j$, then we can safely use the final bid as $b_i + b_j$, so revenue will be very good. This will also naturally consider synergy of pair of ads, etc.
    \sscomment{Can we show that the revenue is always larger? Some assumptions}
\end{discussion}



\paragraph{Computational complexity of BA mechanism}
From the computational perspective, how can one exactly compute the payment function for each $i$?
Essentially, the following procedure shows a way to compute the desired payment for an advertiser.
\begin{enumerate}
    \item Fix $a_1$.
    \item Compute the maximum of \eqref{eq:comb-adjust} for every tuple $A$ that does not include $a_1$.
    \item For every possible tuple $B$ of cardinality $k-1$ that does not include $a_1$, increase $z$ starting from zero and detect the first tuple $a_1 \cup B$ such that the quantity~\eqref{eq:comb-adjust} with $A$ is at least that with $B$.
    \item Charge the computed $z$ to $a_1$. \sscomment{One question here. We adjust $b_1$ to $P(a_1|y_A)$ but still charge $b_1$ - would it be fine? I mean, would it be really smaller than the naive payment~\eqref{eq:comb-naive}. If all the probability $P(a_1 | y_A)$ is just the same, it just becomes naive approach payment.}
\end{enumerate}
\sscomment{Write this down}



\begin{discussion}[Computation of output]
    Disadvantage of~\eqref{eq:comb-adjust} is that it needs to compute the output $y_A$ for every possible $A \in \cA_k$, \ie it requires $\binom{n}{k}$ query to the LLM oracle.
    One alternative way might be to use the probability $\CPr{a_1}{x}$ instead of $\CPr{a_1}{y_A}$.
    \sscomment{Well trained, then concentrated, and then output is not that different? any reference?}
    \sscomment{How much computation latency comparison between $y_A$ and $y_1$? Computation of $P(a_1 |x )$ and $P(a_1 | y_A)$ themselves??}
    \sscomment{Check what is SOTA RAG architecture?}
\end{discussion}

\begin{discussion}[Computation of conditional probability of tuple]
    Also, again from computational perspective, computing $\CPr{a_1,\ldots, a_k}{x}$ for every tuple $A$ is expensive as well, as it requires $\binom{n}{k}$ queries to the similarity oracle.
    So one may use an approximate measure of this quantity.
    A naive approach might be using $\sum_{i \in [k]}\CPr{a_i}{x} / k$, but there is no justification.
    Another one might be a greedily sequential selection.
    For example, we run single allocation mechanism to determine the winner $a_1$.
    Given that $a_1$ is selected, we then determine $a_2$ by considering $\CPr{a_1, a_2}{x}$ as the probability.
    Finally, adjust the bid similar to~\eqref{eq:comb-adjust} and compute the Myerson pricing.
    Research question here might be, would this simple mechanism be good approximation to the above?
\end{discussion}

\begin{discussion}[Computation of payment function]
    Another computational disadvantage of~\eqref{eq:comb-adjust} is that even after we selected the tuple $A$, the computation of the payment function itself also requires at least $\binom{n}{k} \cdot \binom{n}{k-1}$ computation of the quantity~\eqref{eq:comb-adjust}.
    How can we overcome this one?
    For the sequentially greedy selection above, payment computation will be easier, just multiple times of single allocation.
\end{discussion}

\sscomment{We can first compute the ideal deterministic and randomized mechanism theoretically. And then discuss its computational difficulty. Then propose ways to approximate such an ideal mechanism, \ie simple versus optimal mechanism, and investigate what is the approximation of such simple mechanism in terms of social welfare, revenue, etc?}

\sscomment{For experiment: ask LLM to generate ad, and log-normal bid b/w half and one and ctr is random from uniform 0 1. Simulation - compare computation cost, revenue, social welfare, payment, etc.}

\sscomment{Mixture of sequence and token model? At the beginning, one ad and the end, another ad.}



% \krcomment{
% We need to design a function $F$ that takes bids from advertisers and find the appropriate bid for a combination of them. This is a function of original bids, ads from different advertisers, and the original query.
% \begin{align*}
%     F(b_i, b_j, a_i, a_j, x)\CPru{\eta}{a_i,a_j}{x},
% \end{align*}
% A candidate for this function, could use similarity-based approaches that consider the final generation $y_{i, j}$ and compares it with each individual advertisers desires, i.e., $y_i$, and $y_j$. This general apparoach kind of subsumes above models as well. But computing $p(a_i,a_j | x)$ for every pair will be expensive. Heuristic 1: approximate it with $p(a_i |x) + p(a_j | x)$. Heuristic 2: Greedily select $a_i$ and then select $a_j$. Here, we can also have two phase bidding. For example, ask bidders to write first bid, and second bid (when your ad is considered in second round).
% }

\sscomment{Any literature on the combinatorial impact for multiple ad slots?}

\sscomment{For RAG-token, we don't have $\CPru{\eta}{a_i,a_j}{x}$, which probability should we use?}





\paragraph{Randomized mechanism}
\begin{discussion}[Randomized mechanism]
    We can also consider randomized mechanism as well.
\end{discussion}



Basically, we can consider following two types of mechanisms:
\begin{enumerate}
    \item Multi-parameter mechanism: Ask advertisers to write multi-dimensional bids. Basically, write bid for every combination $a_i$ and $a_j$. But this is impractical. Or it might be possible to require advertisers to write each bid for each cardinality of the selected set, \eg for single selection $b_1^{(1)}$, for two selections $b_1^{(2)}$, etc.
    \item Similarity-based adjustment mechanism: Write $b_i$ and decrease it with respect to the similarity relevant measure? It might be more reasonable and simpler for advertiser, however, computationally, winner determination procedure might be heavy.
\end{enumerate}

Let us first focus on approach $2$.
Fundamentally,  we need to design a function $F$ that takes bids from advertisers and find the appropriate bid for a combination of them. This is a function of original bids, ads from different advertisers, and the original query.
\begin{align}
    F(b_i, b_j, a_i, a_j, x, y)\CPru{\eta}{a_i,a_j}{x}, \label{eq:comb-general}
\end{align}
% \sscomment{Shapley share of the original bid? GIven $y_{ij}$, compute Shapley share, and then multiply by bid. Pricing function can be determined by VCG.}

% \sscomment{For paper, define axiom and prove sth? Put the rule, collect advertiser, then dynamics happen, which is hard. So just define theoretical properties, and Toy example in the last section.}


\section{BCK - OLD STUFF}
\subsection{Multiple ads}
\sscomment{Maybe RAG-token model becomes relevant here}
It is not trivial to extend to multiple ads unlike the traditional sponsored search auction.
This is mainly because the output is not structured, \ie not a series of available slots, and also incorporating multiple ads affect each other in LLM ads.
How can we cope with it?

\paragraph{Allocation function}
We further might be able to retrieve multiple ads at once.
Essentially, given that a set of ads $A$ is retrieved, we have
\begin{align}
    \CPr{y}{x} = \sum_{A \subset \cA} \CPru{\eta}{A}{x} \CPru{\theta}{y}{x,A} \, .
\end{align}

Suppose that we want to advertise a fixed number of ads $k$ per each query.
Then the constraint for $A$ is $|A| = k $, and the corresponding probability distribution will be

\begin{align}
    \CPr{y}{x} = \sum_{A \subset \cA: |A| = k} \CPru{\eta}{A}{x} \CPru{\theta}{y}{x,A} \, .
\end{align}

\paragraph{Bidding mechanism}
If multiple ads are incorporated in a single output, it might be the case that the impact of the advertisement for each ad decreases.
So, each advertiser $i$ may not want to pay the full bid $b_i$ in this case.


What will be then reasonable bidding mechanism here?
A simple approach might be if ad $a_1$ and $a_2$ is merged, then use $(b_1 + b_2)/2$.
This is unfair if the final output is geared towards $2$ for example.

What will be the difference in the advertisement effect on $1$  compared to the case when only $1$ is advertised?
It is basically how $a$ fits into the original query.
So
\begin{align*}
    \CPru{\eta}{a_1}{x}
\end{align*}
versus
\begin{align*}
    \CPru{\eta}{a_1, a_2}{x}.
\end{align*}
So we may consider $a_1$'s bid as 
\begin{align*}
    b_1 \cdot \frac{\CPru{\eta}{a_1, a_2}{x}}{\CPru{\eta}{a_1}{x}}.
\end{align*}
Q: what if this weight is actually larger than $1$? This means that the context becomes more relevant by incorporating $a_2$ as well, but the overall advertisement effect might be distributed as two products are advertised. A simple approach might be to cap by $1$.

\sscomment{
Also such a bidding rule should be reasonable so that advertisers agree on the contract. 
More mechanism design style of requestions below in the payment function paragraph.
}


\paragraph{Sampling}
Then how can we sample from the desired target distribution above?
This might be similar to the case of single ad.
We basically change the single ad into multiple ones.

But, in a computational perspective this might not be tractable.
This is because in the single-ad case we only need to create output samples for each $a$, and the draw one of them.
With multiple ads here, we should create output samples for each $A$, and draw one of them.
Technically the number of sample here can be $\binom{n}{k} = \Theta(n^k)$, which is polynomial given that $k$ is polynomial but can be heavy given the very restricted response time for ad auction.

\begin{question}
    So one question might be how to efficiently sample from it.
\end{question}

A naive approach might be to use a hardmax rule with greedy selection.
For example, pick any ad $a_1 \in \cA$. For $a \in \cA \setminus \{a_1\}$, pick $a_2$ by looking at the distributions $\CPru{\eta}{a_1}{x,a}$, $\CPru{\eta}{a}{x}$, or any other relevant information that one may use.
Repeat for some $k$ iterations.

\paragraph{Payment function}
What should be the total payment to $A$? Probably based on the payment rule by Myerson.
How should we share the payment among $A$? 
Basically we should design payment function and corresponding bidding mechanism to be \emph{incentive compatible} while implementing the allocation function.

Aside from the incentive compatibility and bidding mechanism, let's just think about what happens if there were no $a$ in $A$.
Then, the allocation probability will be 
\begin{align}
    \CPru{\eta}{A \setminus \{a\}}{x} \, .
\end{align}
So, a marginal contribution of $a$ to $A$ will be
\begin{align}
    \CPru{\eta}{A}{x} - \CPru{\eta}{A \setminus \{a\}}{x} \, .
\end{align}
However, the summation over the marginal contributions do not sum up to $\CPru{\eta}{A}{x}$.

Alternatively we can consider Shapley value as follows to account for the marginal contribution of $a$ marginalized for every possible subsets.
\begin{align}
    \phi_a = \frac{1}{n} \sum_{S \subset A \setminus \{a\}} \frac{\CPru{\eta}{S \cup \{a\}}{x} - \CPru{\eta}{S}{x}}{\binom{n-1}{n-|S|-1}} \, .
\end{align}
An advantage is that this sums up to the original function.
\begin{align}
    \CPru{\eta}{A}{x}  = \sum_{i \in A}\phi_a \, .
\end{align}
Importantly, however, note that $\phi_i$ can be negative sometimes as the following is not always positive:
\begin{align}
    \CPru{\eta}{S \cup \{a\}}{x} - \CPru{\eta}{S}{x} \, .
\end{align}

\sscomment{The notion of core and Shapley value and their usage is different from the standard cooperative game theory. In the standard game theory, Shapley value is a payment function that satisfies a reasonable set of properties, and Core is a payment function that satisfies strategy-proofness in the grand coalition. Here, we are interested in whether agent $i$ will truthfully bid $b_i$ but not about whether $i$ will cooperate with some others, etc. }

\begin{question}
    What will be reasonable pricing scheme for each ad $a$ in $A$?
    Which payment function \& bidding mechanism would guarantee reasonable set of desiderata: incentive-compatibility, individual rationality, etc.
\end{question}

\paragraph{Framework by~\cite{duetting2023mechanism}}
Ad $a$ desires the distribution $\CPru{\theta}{y}{x,a}$ and its bid is $b_a$.
We can use the aggregation function and payment function proposed by~\cite{duetting2023mechanism}.
This way, it naturally combines multiple ads at once.

\begin{question}
    As can be seen from the experiment in~\cite{duetting2023mechanism}, this way of aggregation might not work well if there exists competitive ads (substitutes) since they may not want to be advertised together. One may again need to preprocess the set of ads $\cA$ to handle this kind of issue.
    We can conduct an experiment on how their aggregation function works in case of substitutes and complements (ads with synergy).
\end{question}

\begin{question}
    Also it might be better to select just a few ads and aggregate them afterwards instead of trying to aggregate all the preferred distributions.
\end{question}


what is the summation of welfare of the others when $i$ does not exist?
Let $\cA_k^{-i} = \{A \in \cA: i \notin A, |A| = k\}$.
Among $A \in \cA_k^{-i}$, define $A'$ as follows.
\begin{align*}
    A' = \argmax_{A \in \cA_k^{-i}} k \cdot f(d_A) + \sum_{j \in A} q_{A,j}b_j.
\end{align*}

Then, we have the social welfare of the others when $i$ is not present as follows.
\begin{align*}
    \SW^{-i} = 
    \sum_{j \in A' }  q_{A',j} b_j +  f(d_{A'}).
\end{align*}

\begin{align*}
    \SW - u_i = 
    \sum_{j \in A^* \setminus \{i\}}  q_{A,j} b_j +  f(d_{A^*}).
\end{align*}

Thus, $a_i$'s externality is 
\begin{align*}
    \Ext_i 
    &= \SW^{-i} - (\SW - u_i)
    \\
    &=
    \left( \sum_{j \in A'}  q_{A',j} b_j +  f(d_{A'}) \right)
    - 
    \left( \sum_{j \in A^* \setminus \{i\}}  q_{A,j} b_j +  f(d_{A^*}) \right).
\end{align*}




    % This is not single-dimensional mechanism, so we cannot ground on the Myerson's lemma~\ref{lem:myerson}. \SLcomment{Why isn't this a single-dimensional mechanism? Each ad still just has a single parameter $b_i$ (and valuations are single-parameter).}
    
    % \sscomment{That is because we assume that each bidder's true valuation is in fact $v_i \cdot q_{A,i}$ given that a set of ads A is allocated for $i \in A$. So, it is essentially analogous to each bidder writes multi-dimensional bids for every possible combination $A$. Since that is impractical, we impose the assumption on the relevance based valuation, and simply ask bidders to write a single bid. 
    
    % This is in fact analogous in the single allocation setting, since ideally we can ask bidders to write bid for every possible output $y$, \ie $b_i = b_i(y)$. The reason that Myerson works there is that, the advertiser's true valuation is still a single value given any output (although it depends on the output). For example, for ad $a_i$, if $y_i$ is chosen, then it is $q_i \cdot v_i$, and otherwise, it is $0$. On the other hand, each bidder faces multiple different valuation based on what other ads are selected in $A$ for this multi allocation setting, so we cannot use Myerson.} \SLcomment{I'm still not convinced, maybe we'll have to discuss in person. In $v_i q_{A,i}$, the space of valuations is still determined by the single scalar $b_i$, which makes it a single-dimensional type space. If you evaluate Myerson's formula, you should see that you recover the VCG payment scheme here.}
    % \sscomment{I see. I think you are right! I was confused. This is actually Myerson payment as well. I will fix the presentation/computation here.}
    % Instead, we use the VCG mechanism~\cite{roughgarden2010algorithmic}.
    
% Running a first-price auction yields that $x$ allocates $1$ to the ad $a^*$ with highest revenue, \ie $x_i = 1$ only if $a_i = \argmax \Rev_{a_i}$ and the corresponding payment is $b_a$.







\section{Further questions}
\subsection{Mechanism for CPC}
\paragraph{Payment function}
In the simplistic setting of~\eqref{pr:1}, the probability that the ad $a$ is retrieved given $x$, \ie $\CPru{\eta}{z}{x}$, provides an indirect measure of how relevant the ad $a$ is to the query $x$.
Say we have a mapping $f:\R \to \R$ that maps $\CPru{\eta}{z}{x}$ to the ground truth click-through-rate (CTR).
Let $b_a$ be the bid of ad $a$, assuming that all the ads are registered as cost-per-click (CPC) model.

Then the expected revenue from delivering $z$ can be computed as
\begin{align}
    \textsc{Rev}_a = b_a \cdot f(\CPru{\eta}{a}{x}).
\end{align}
\sscomment{Starting from just probability, we can update it via training. Training is not straightforward though.}
\sscomment{$y$ is related to the CTR as well. Impression?}

\sscomment{Cost-per-impression world. Consider how to incorporate the probability into the bids. Viewability.}
\sscomment{STart with that probability of $p(a|x)$ and adjust based on the ratio of bids. Loglinear aggregation from Renato's paper}
% \sscomment{So, in case of retrieving a single ad, it might be sufficient}


\subsection{Retrieve with documents}
We may need to retrieve a pair of (ad, document) to make it more relevant to the original query $x$ as follows.

\begin{align}
    \CPr{y}{x} = \sum_{a \in \cA, d \in \cD(x)} \CPru{\eta}{a,d}{x} \CPru{\theta}{y}{x,a,d} \, .
\end{align}

\begin{question}
    What about if we want to make the output more relevant to the document than advertisement?
    Is there any relevant paper?
\end{question}





----------------------------------------


We construct a mechanism to run an ad auction in the output of the LLM, \eg along in the text.\footnote{\sscomment{This might decrease the user's satisfaction, however, as discussed in~\cite{feizi2023online}, the platform may attach hyperlinks to explicitly let the users know that the certain parts are constructed from ads, similar to the standard sponsored search auction.}}
\sscomment{Discuss how it differs from the standard search auction design}

We are interested in the standard single-dimensional mechanism with quasi linear utility.

\subsection{Output selection}
\sscomment{Define LLM and similarity oracle here.}
A set of advertisements $\cA = \{1,2,\ldots,n\}$ is given.
% Write $\cD(x) =\textsc{TopK}(\CPr{\cdot}{x})$ to denote the top k documents given $x$.
In the RAG-Sequence model, the probability is computed as
\begin{align*}
    \CPr{y}{x} = \sum_{z \in \textsc{TopK}(\CPr{\cdot}{x})} \CPru{\eta}{z}{x} \CPru{\theta}{y}{x,z} \, 
\end{align*}
Suppose that we replace the documents with the advertisements, then we obtain.
\begin{align*}
    \CPr{y}{x} = \sum_{a \in \cA}\CPru{\eta}{a}{x} \CPru{\theta}{y}{x,a} \, .
\end{align*}
Since we are firstly interested advertising a single product given a query, we may choose an ad $a$ and then compute
\begin{align}
    \CPr{y}{x} = \CPru{\eta}{a}{x} \CPru{\theta}{y}{x,a} \, .\label{eq:single}
\end{align}
Fundamentally, once an ad $a$ to advertise is determined by a mechanism, we will sample the output $y$ based on~\eqref{eq:single} and display the eventual output $y$.
Precisely, as per~\cite{lewis2020retrieval}, in the decoding time we should select the output $y$ that maximizes
\begin{align*}
    y = \argmax_{y} \CPr{y}{x}.
\end{align*}
Note that this can be approximated by \emph{thorough decoding} or \emph{fast decoding} proposed in~\cite{lewis2020retrieval}.




\subsection{Mechanism}
Basically we will use the probability vector $\CPru{\eta}{a}{x}$ for each $a \in \cA$ to obtain our final ad allocation vector.
For simplicity assume that all the advertisers are charged based on cost-per-impression (CPM).
% Overall, the mechanism $\Mec$ defines an allocation function $x: (\R^2)^n \to [0,1]^n$ that maps the sequence of pair of bid and CTR to the probability vector over $n$-dimensional simplex, and a payment function $p: (\R^2)^n \to \R_{\ge 0}^n$ that maps to the payment for each advertiser.
Given $n$ advertisers, let $X \subset \R^n$ be the set of feasible allocations for the advertising auction.
For example, in case only a single ad is served, $X$ will be a probability simplex over $\R^n$.
Write $q_a = \CPru{\eta}{a}{x}$ for $a \in \cA$.

To discuss several properties of the mechanism, it is essential to rigorously define the notion of the advertiser's valuation.
For ease of exposition, we start with the simplest setting in which each advertiser is only interested in being selected and appearing in the LLM output regardless of the quality of it.
That is, the advertiser $i$ is willing to write bid $b_i$ consistently for being selected in the output.
\begin{assumption}[Valuation]\label{as:naive-valuation}
    Advertiser $i$'s private valuation for being selected and advertised in any output $y$ is $b_i$.
\end{assumption}
Since the advertiser may want to write complicated bids based on the quality of the output and relevance of the ad to the query, we tackle the assumption above in Section REF.

\begin{definition}[Mechanism]
    A mechanism $\Mec = (\x, \p)$ is fully specified as follows.\footnote{In fact, one may think about indirect mechanism possibly with multiple communication, but the revelation principle by~\cite{myerson1981optimal} asserts that it is without loss of generality to consider the class direct mechanism as we defined.}
    \begin{enumerate}
        \item Collect bids $\b = (b_1,\ldots, b_n) \in \R^n$.
        \item Compute baseline probability vector $\q = (q_1,\ldots, q_n) \in \R^n$ according to~\eqref{eq:single}.
        \item {\bf Allocation rule}: A feasible allocation vector $\x(\q, \b) \in X$
        \item {\bf Payment rule}: payments $\p(\q, \b) \in \R^n$
    \end{enumerate}
\end{definition}

Given the allocation rule, advertiser $i$'s utility can be defined as
\begin{align*}
    u_i(\q, \b) = v_i \cdot x_i(\q, \b) - p_i(\q, \b),
\end{align*}
where $v_i$ denotes advertiser $i$'s true private valuation of being advertised.
We often write $b_{-i}$ to denote $(b_1,b_2,\ldots, b_{i-1},b_{i+1}, \ldots, b_n)$ and similarly for $x_{-i}$ and $p_{-i}$.

\begin{definition}[Equilibrium]
    Given a mechanism $\Mec = (\x, \p)$, the bidding strategies $\b$ is a Nash equilibrium if $u_i(\q, \b) \ge u_i(\q,\b')$ where $b' = (b_i', b_{-i})$ for every $i \in [n]$.
    If $u_i(\q, \b) \ge u_i(\q, \b')$ for every $i \in [n]$ regardless of the choice of $b_{-i}$, then it is a dominant strategy equilibrium.
\end{definition}

We are essentially interested in a mechanism that has the truthful reporting as a dominant strategy equilibrium.
\begin{definition}[DSIC]
    A mechanism $\Mec = (\x, \b)$ is dominant-strategy incentive-compatible (DSIC) if truthful bidding is a dominant strategy for every advertiser $a \in \cA$.
\end{definition}


% We further define several notations to introduce the seminal result by~\cite{}
According to the seminal result by~\cite{myerson1981optimal}, there exists a unique payment rule to implement any monotone allocation function, where monotonicity and implementability of an allocation function is formally defined as follows.
% To this end, we first need to define the definition of implementable allocation rule along with several other notations.


% \begin{definition}[DSIC]
%     A mechanism $\Mec = (\x, \b)$ is dominant-strategy incentive-compatible (DSIC) if truthful bidding is a dominant strategy for every advertiser $a \in \cA$.
% \end{definition}

% Our main objective is to characterize DSIC mechanism with desirable allocation rule, to meet the user satisfaction as well as the advertiser's utility and the platform's revenue.

\begin{definition}[Monotonicity and implementation]
    An allocation rule $\x$ is monotone if the function $x_i(z ; b_{-i})$ given $b_{-i}$ is nondecreasing in $z$.
    Further, $\x$ is implementable if there exists a corresponding payment rule $\p$ such that $\Mec = (\x, \p)$ is DSIC.
\end{definition}

% The seminal result by~\cite{myerson1981optimal}


% \begin{definition}[Implementation]
    
% \end{definition}

Then Myerson's lemma can be written as follows.
\begin{lemma}[\cite{myerson1981optimal}]
    Consider a single-parameter auction environment.
    \begin{enumerate}
        \item An allocation rule $\x$ is implementable if and only if it is monotone.
        \item If $\x$ is monotone, then there exists a unique payment rule $\p$ such that $\Mec = (\x, \p)$ is DSIC assuming that $p_i(\b) = 0$.
        \item The payment rule is given by
        \begin{align}
            p_i(b_i, \b_{-i}) = \int_{0}^{b_i} z \cdot \frac{d}{dz} x_i(z, \b_{-i}) dz \, .
        \end{align}
    \end{enumerate}
\end{lemma}


It is worth noting that the mechanism above does not maximize the social welfare per se since it does not allocate the ad $a$ with highest valuation $b_a$, but to the highest weighted valuation $q_a b_a$.
In fact, 
\sscomment{Mention that $q_a$ is a proxy for CTR in the model section.}
    
    
    One may think of this as the mechanism maximizing a \emph{weighted social welfare} in a sense that the valuation of each ad is adjusted to be $q_a \cdot b_a$ rather than $b_a$, and we allocate
    This would be reasonable for the advertisers as well since if $q_a$, \ie the relevance, is significantly low, then the advertiser's true valuation in hindsight might be much lower than just $b_a$.


\begin{discussion}
    This can be viewed as maximizing social welfare if the advertiser's utility is in fact $u_i(\q,\b) = q_i v_i \cdot x_i(\q,\b) - p_i(\q,\b)$ instead of~\eqref{eq:adv-util}, where the resulting social welfare will be equivalent to the efficiency.
    Indeed, if one assumes that the advertiser's true valuation is $q_i v_i$ instead of $v_i$, then the advertiser's utility will be $q_iv_i$ if it is selected by the mechanism.
    One may interpret the advertiser $i$ writing the bid $b_i$ as committing to the relevance-based bidding contract in a similar vein to the autobidding, \eg~\cite{lucier2023autobidders}, so that the bid will be close to $b_i$ if the relevance is higher and vice versa.
    \sscomment{We can more emphasize this.}
\end{discussion}

\begin{discussion}
    Alternatively, one may think about the efficiency as an objective that accounts for the user's utility as well.
    For example, suppose that user's utility is exactly proportional to the relevance $q_i$, \ie $u_{user}(\q, \b) = \theta \cdot q_i$.
    Then, maximizing $\q \cdot \x$ is equivalent to maximizing $\log(u_{user}(\q,\b)) + \log(\SW)$, which is the log linear summation of the user' utility and the social welfare.
    This is also related to the $\alpha$-fairness notion by~\cite{lan2010axiomatic}, where the social utility is defined by $\sum_i u_i^{1-\alpha}/ (1-\alpha)$, and letting $\alpha \to 1$ yields maximizing the product of the utilities.
\end{discussion}


\subsection{Randomized mechanism with softmax allocation}
\sscomment{Pros and cons? may have benefit for risk-averse bidders. but for revenue maximizing purpose, it seems deterministic mechanism is better.}
If all the advertisers write the same bids for their ads, we can allocate each ad $a$ with probability $q_a$ as in the original RAG-sequence model.
Note however that if $X$ is a probability simplex over $\R^n$, then we need to normalize the summation such that
\begin{align*}
    x_a(\q,\b) = \frac{q_a}{\sum_{i \in \cA} q_i}.
\end{align*}



\begin{theorem}
    Consider RAG-based LLM advertising auction with base probability $\q$ and bids $\b$.
    The following mechanism $\Mec$ is DSIC:
    \begin{align}
        \Mec = (\x, \p) = \left( \frac{q_a b_a}{\sum_{i \in \cA} q_i b_i}, \frac{w}{q_a} \parans{\frac{w}{w + q_ab_a} - 1 - \ln \frac{w}{w+ q_ab_a}} \right) \, .
        % \label{eq:single-rand-mec}
    \end{align}
\end{theorem}



\paragraph{Design choice}
Further things to discuss:
\begin{enumerate}
    \item Alternative baseline probability: One may use probability $\CPru{\eta}{a}{y,x}$ to run the auction instead of $\CPru{\eta}{a}{x}$.
    Note first that each ad $a$ will incur a different distribution over possible $y$.
    Basically if we incorporate $y$, then there might be a case that even though both $y$ and $a$ are (relatively) irrelevant to $x$, but it happen to have high $\CPru{\eta}{a}{y,x}$.
    On the other hand, incorporating $y$ makes the probability much more relevant to the actual output, so it might be helpful to identify the real correlation between the ad and the output.
    \sscomment{Computationally incorporating $y$ becomes much much more expensive.}
    \item Thresholding: In case the ads are very irrelevant to the query, we should avoid advertising it.
    Essentially we can implement a threshold for the allocation probability $\CPru{\eta}{a}{x}$. 
    \sscomment{similar to top k or up to top k? top k with $q$ and then incorporate $b$? Threshold plus top k.}
    % \item Sampling: How to sample the eventual output $y$ given the weights from the desired distribution?
    % Essentially we can draw multiple (w.r.t. $b_a$ and $\CPru{\eta}{a}{x}$) samples for each document and randomly draw one of them. 
    \item Computing $y$: we need somehow approximation for $\argmax_y p(y|x)$ similar to~\cite{lewis2020retrieval}.
    \item Further allocation vector can be used, similar to the sampling algorithm in \href{https://towardsai.net/p/machine-learning/how-does-an-llm-generate-text}{link}.
    \item Advertisers may want to have complicated bidding function based on the context of the query.
\end{enumerate}

\sscomment{todo: how about RAG-token model?}

==> model.tex <==
TODO list for the draft
\begin{enumerate}
    \item Fix notation (valuation $v_i$, bid $b_i$). Do not use subscript $a$ as it's confusing with ad $a_i$. Also $\x$ is confusing with $x$.
    \item Polish model section
    \item Make sure to emphasize LLM
    \item Make sure that in practice, ad url can be inserted whenever ad is there, which explicitly hints that is sponsored ad. \sscomment{Whenever advertiser's brand name is written, we can explicitly add link.}
    \item Check if our model subsumes CTR valuation model, \ie when $v_i$ is the valuation of the click, and relevance is an indirect measure of CTR.
\end{enumerate}


\sscomment{Intro: inspired by RAG. In the mmodel, generla.}




%%
%%

\section{Outline}

- segment-wise mechanism, single-ad per segment
    - do we condition next-segment generation on previous-segment generation?
    - discuss using final output to evaluate allocation probabilities
- what does the allocation rule optimize? what welfare function?
    - linear aggregation (Nash social welfare)
    - log-linear aggregation
    - if all bids are the same, revert to baseline RAG selection probabilities
- what is the truthful payment rule?
    - discussion of charging per click
- multi-ad allocation per segment
    - discussion of using final output to evaluate allocation probabilities, extra queries

For user experience: briefly discuss thresholded rule, etc.



Design dimensions that can vary:
\begin{itemize}
    \item Number of times ads are selected and allocated during output generation: e.g., every sentence, paragraph, section, etc.
    \item Number of ads selected for each segment: single or multiple.
    \item Aggregation function used to aggregate baseline ad selection probabilities according to bids: linear, log-linear.
    \item Pricing schemes for the auction:
        \begin{itemize}
            \item Truthful (unique)
            \item Next-highest bid
        \end{itemize}
\end{itemize}

Theory questions:
\begin{itemize}
    \item For each aggregation function, what social welfare function is it implicitly maximizing?
    \item What is the characterization of the truthful payment scheme for RAG?
\end{itemize}


Simulation set up:
\begin{itemize}
    \item 
\end{itemize}


Empirical questions:
\begin{itemize}
    \item How close is "next-highest bid" pricing to truthful pricing?
\end{itemize}



%%
%%

\section{Mechanism Design for LLM Advertising}

\subsection{Problem setup}
% Given a LLM, let $\Theta$ be the set of every possible tokens and $\Theta^*$ be the set of finite sequences over $\Theta$.
We here formally define the mechanism design problem for LLM advertisement auction.
Overall, we are interested in a mechanism to determine which ad to select, how much to charge the advertiser, and how to construct the eventual output $y$ that will be shown to the user as a response.

Precisely, consider a set of advertisement (ad) $\cA = \{1,2,\ldots, n\}$ is given where each ad is equipped with an advertiser.\footnote{In practice, a single advertiser may run multiple ads. Our model subsumes this scenario by allowing the same advertiser across different ads in $\cA$. However, we assume that the advertiser simply strategizes its bid over each single ad instead of combinatorically deciding the entire bids. TODO: Double Check}
We often write $a_i$ to denote $i$-th ad for clarity.
Before the platform runs, each advertiser $i$ writes a bid $b_i$ based on its true valuation $v_i$.
Formally, we assume that each advertiser $i$ is equipped with a private valuation $v_i$ for being selected and advertised in any output $y$.\footnote{Since the advertiser may want to write different bids based on the quality of the output and relevance of the ad to the query, we relax this definition of true valuation to make our model more practical at paragraph \emph{Social Welfare} in Section~\ref{subsec:desiderata}}

% \begin{definition}[Valuation]\label{as:naive-valuation}
%     Advertiser $i$'s private valuation for being selected and advertised in any output $y$ is $v_i$.
% \end{definition}

At each round, a user arrives in the LLM platform, and writes a query $x$ to the LLM.
Given the query $x$, the set of ads $\cA$, and the bids $\b = (b_1,b_2,\ldots, b_n)$, a mechanism should determine which ad $a_i$ to advertise as well as how to constitute the output given $a_i$ and $x$.

At a first (and naive) glance, we may simply run the standard second price auction (or first price auction) given $\b$ as the bids.
This approach, however, may significantly decrease the user satisfaction given the query $x$, since there might be a scenario that none of the ads in $\cA$ is relevant to the query $x$ in hindsight.
Fundamentally, there should be a measure for each ad $a_i$ to estimate how it can well be incorporated in the output without hurting the context too much.

To this end, we assume that we have an access to a relevance oracle, formally defined as follows.
\sscomment{Incorporate $y$ here, then in the discussion, skipping $y$ makes efficiency. Rename it.}
\begin{definition}[Relevance oracle]\label{def:rel-orc}
    A relevance\footnote{Such kind of measure is called as a \emph{quality score} in~\cite{qualityscore}, and plays a key role in the search ad, \eg see~\cite{aiello2016role} and~\cite{hillard2010improving}.} oracle $r(a_i | x)$ computes a nonnegative real number $q_i \in [0,1]$ that represents the relevance of the ad $a_i$ given the query $x$.
\end{definition}
Notice that we implicitly assume a normalization by scaling $q_i$ to fall within the unit interval $[0,1]$.
In practice, this can be implemented by \sscomment{Keivan: write sth about embedding, etc}.




\begin{discussion}\label{dc:relevance-ctr}
    Alternatively, one may view the relevance $r(a_i|x)$ as a substitute of the click-through-rate (ctr) in the standard sponsored search auction.
    Indeed, in the sponsored search auction, the CTR is used as a proxy of the impact of the advertisement, and in our LLM auction, the relevance will be highly related to the impact of the advertisement in LLM auction correspondingly.
    \SLcomment{I don't really agree with this. The CTR will also depend on the final output $y$. I see the relevance here as analogous to the document selection probability $p_{\eta}(z | x)$ in the RAG paper. Actually you mention that connection below. I think the CTR should be a separate function, that takes in the final output and maps to a CTR for an ad.}
    \sscomment{I see your point I think we can skip this discussion. Actually, as mentioned in Section~\ref{sec:single-further-disc}, it may become relevant if we consider relevance measure as a function of $y$ as well. But it might not be worth discussing it here.}
\end{discussion}



Assuming that the mechanism have selected an ad to advertise along in the LLM's response, we consider there also exists a black-box module that computes the desired output, formally defined in the following.
\begin{definition}[LLM oracle]
    A LLM oracle $l(a_i, x)$ constructs the response $y_i$ consisting of a sequence of tokens that incorporates the ad $a_i$ in the response to the query $x$.
    \SLcomment{I see this as analogous to the $p_{\theta}(y | x, z) = \prod_{t=1}^T p_{\theta}(y_t | x, z, y_{1:t-1})$ generative probabilities in RAG.}
\end{definition}
From the practical perspective, a description of the ad $a_i$ can be appended following $x$ in a prompt-engineering manner to implement such a module.
Note that this is similar to the philosophy of \emph{retrieval-augmented generation} (RAG) for LLM by~\cite{lewis2020retrieval}.
Indeed, each ad $a_i$ can be considered as a document $z_i$ in the RAG framework.
Interestingly, then, the conditional probability $\CPr{z}{x}$ of retrieving the document $z$ given $x$ can be thought of as our relevance oracle $r(a_i | x)$.\footnote{One may consider a relevance oracle to receive the outcome of the LLM oracle $y_i$, \ie $q_i = r(a_i, y_i | x)$, but a sophisticated choice of the relevance oracle may already subsume this setting since $y_i$ itself is again a function of $a_i$ and $x$. In addition, if the LLM module (oracle) is well-implemented, one may expect that the relevance of $a_i$ given $x$ is close enough to the relevance of $a_i$ given $y_i$ and $x$ since there would be a strong correspondence between $x$ and $y_i$ given $a_i$.}
\sscomment{We can expand a bit more in the appendix, if worth}

Having defined the necessary modules to run LLM ad auction, the overall timing of the mechanism can be formally defined as follows.


\begin{definition}[Mechanism]
    Given the relevance and LLM oracle, a mechanism $\Mec = (\x, \p)$  can completely be characterized as follows.\footnote{One may think about indirect mechanism possibly with interactive communication, \eg English auction, but the revelation principle by~\cite{myerson1981optimal} asserts that it is without loss of generality to consider the class of direct mechanisms.}
    \begin{enumerate}
        \item Collect bids $\b = (b_1,\ldots, b_n) \in \R^n$ from the advertisers.
        \item Compute the relevance $\q = (q_1,\ldots, q_n) \in \R^n$ from the relevance oracle.
        \item {\bf Allocation rule}: An ad is selected according to the allocation function $\x(\q, \b) \in \Delta_n$ where $\Delta_n$ denotes $n$-dimensional probability simplex.\footnote{A deterministic mechanism necessitates that the resulting allocation vector $\x$ is a unit vector. A allocation vector that is not a unit vector can be thought of as a randomization over the deterministic mechanism.}
        \item {\bf Payment rule}: Advertisers are charged based on the payment function $\p(\q, \b) \in \R^n$.
        \item LLM oracle constructs the final output $y_i = l(a_i, x)$ given that $a_i$ is selected above.
    \end{enumerate}
\end{definition}
Mainly, our objective is to design an allocation function $\x$ and a payment function $\p$ that satisfies several desiderata which will be discussed shortly.
\SLcomment{
How does this map to RAG? Here are some thoughts. Write the selection probability in RAG given bids as $p_{\eta}(z_i | x; \b)$. This should be a monotonically increasing function of $b_i$, and if all bids are the same we should have $p_{\eta}(z_i | x; b_i) = p_{\eta}(z_i | x)$, i.e., the initial probabilities before modification by bids.

Under RAG-Sequence we have
$$
p(y|x) = \sum_{z \in \mathrm{top-k}(p(\cdot|x;\b))} p_{\eta}(z | x; \b) p_{\theta}(y | x, z)
$$

Taking inspiration from the "LLM Summaries" paper (Aranyak's paper), it makes sense to relate the CTR of ad $i$ given output $y$ to its "prominence" in the output. One measure of prominence could be the posterior:
$$
p(z_i | x, y; \b) \propto p_{\eta}(z_i | x; \b) p_{\theta}(y | x, z_i)
$$
(Motivated by Figure 2 in the RAG paper that shows how the posterior can intuitively assign a document to each token generated.)

We could assume that the CTR of ad $i$ is monotonically increasing in the ad's prominence:
$$
CTR_i(p(z_i | x, y; \b)) = CTR_i(p_{\eta}(z_i | x; \b) p_{\theta}(y | x, z_i))
$$
(the latter isn't quite right, it depends on all the ads' posteriors due to the normalization.)

The fact that that $p(z_i | x, y; \b)$ is increasing in $b_i$ follows from the fact that $p_{\eta}(z_i | x; \b)$ is increasing in $b_i$.

The advertiser's utility for the resulting output is $v_i CTR_i(p(z_i | x, y; \b)) - p_i(\cdot)$.

A few comments/questions:
\begin{itemize}
    \item The form of the IC payment rule needs to be worked out, and it needs to be implemented somehow in practice (e.g., how do we compute the integral in Myerson's formula)
    \item What objective is this kind of allocation optimizing for? (how does it trade-off advertiser and user utility)
\end{itemize}

The assumption that CTR is monotonically increasing in the prominence (posterior) may be too strong or not justified. Suppose that the LLM output never depends on the selected doc for some reason:  $p_{\theta}(y | x, z_i) =  p_{\theta}(y | x)$ (for example, there may be a bug in how the prompt is put together, and the doc info just gets dropped). Then the posterior is just the prior: 
$p(z_i | x, y; \b) = p_{\theta}(y | x, z_i)$. But it doesn't make sense for CTR to be increasing on just the prior: if the final $y$ output doesn't depend on the doc and its bid, there is no way the CTR for the ad to change.
}

\sscomment{I think this would be good points to spell out, \eg how our model subsumes such kind of interpretation?
One question: what would $p(z | x ; b)$ actually look like? Our original version seems to be using $p(z | x) \cdot b$, so are you thinking of any function $f(p(z|x), b)$?}
\SLcomment{Renato's paper has two examples of $p(z|x;\b)$, and there may be other interesting ones. One of their examples is indeed using $p(z|x;b)$ (renormalized). The other is to weigh the log probabilities by bids, and renormalize.}

\sscomment{I'm not very sure how $p_{\theta}(y | x,z)$ and posterior can be obtained, but doesn't it require that we have trained entire RAG LLM given the static set of ads, which is not practical? In our approach, once the ad to advertise is selected via a mechanism, we simply condition on that ad by prompt engineering, and then generate output, which does not require to retrain the system.} \SLcomment{Yes, we could define $p(y|x,z)$ however we like (so maybe I should have dropped the $\theta$ parameter). The RAG paper trains it, but a simpler way is just to append $z$ to the prompt, i.e., prompt engineering just as you said.}

\sscomment{
To interpret it in our model's perspective a bit more precisely:
We have $p(z | x ; b) = p(z | x) \cdot b_i$, i.e. relevance times bid.
As mentioned above, we first run a mechanism to select which ad to show, and condition on that ad, then generate the output.
Further, we just use the same relevance to model CTR, \ie $p(z | x ; b)$ instead of $p(z | x,y ; b)$.
In fact, we can generalize our original setting to have another oracle measure which is a function of $y$ as well to capture $p(z | x,y ; b)$.
Given that, we assume that advertiser's valuation is $v_i \cdot CTR$ (Definition 1.13), so this is also analogous.
So, advertiser's utility is $v_i \cdot CTR - payment$ which corresponds to $v_i * q_i - p_i$ in our setting.
Then, the mechanism can analogously be derived.
One difference is that if we define $CTR$ to be a function of $y$ as well, we will need to precompute $y_i$ for every ad $a_i$ and then run the mechanism as discussed in Section~\ref{sec:single-further-disc}. (this is not that circular as I commented on that section.)
}

Given a mechanism $\Mec(\x, \p)$, the advertiser $i$'s utility can be written as
\begin{align}
    u_i(\q, \b) = v_i \cdot x_i(\q, \b) - p_i(\q, \b),\label{eq:adv-util}
\end{align}
where $v_i$ denotes advertiser $i$'s true private valuation of being advertised.
When we deal with randomized mechanism, we take expectation in the right hand side.
% \sscomment{Not sure if the current presentation will be the best}



Furthermore, the mechanism designer's utility, \ie revenue, from $\Mec$ will be defined as
\begin{align*}
    \Rev = u_{\Mec}(\q, \b) = \sum_{i \in [n]} p_i(\q, \b).
\end{align*}
We often write $\b_{-i}$ to denote $(b_1,b_2,\ldots, b_{i-1},b_{i+1}, \ldots, b_n)$ and analogously for $\x_{-i}$ and $\p_{-i}$.


\subsection{Desiderata}\label{subsec:desiderata}
\paragraph{Truthfulness}
To elaborate on our results, we present preliminaries on the mechanism design literature.
First, the mechanism's characteristics will be analyzed on its equilibrium.
\begin{definition}[Equilibrium]
    Given a mechanism $\Mec = (\x, \p)$, the bidding strategies $\b$ is a Nash equilibrium if $u_i(\q, \b) \ge u_i(\q,\b')$ where $\b' = (b_i', \b_{-i})$ for every $i \in [n]$.
    If $u_i(\q, \b) \ge u_i(\q, \b')$ for every $i \in [n]$ regardless of the choice of $b_{-i}$, then it is a dominant strategy equilibrium.
\end{definition}

Moreover, we are essentially interested in a mechanism that has the truthful reporting as a dominant strategy equilibrium.
\begin{definition}[DSIC]
    A mechanism $\Mec = (\x, \b)$ is dominant-strategy incentive-compatible (DSIC) if truthful bidding is a dominant strategy for every advertiser $a \in \cA$. We often say the mechanism is truthful.
\end{definition}

\SLcomment{One of the challenges in defining this model has been to come up with reasonable utility functions for LLM output, given an ad. It occurred to me that scoring rules might be useful here. A scoring rule $S(p, y)$ in our context would take in a distribution over output tokens (or output sequences) $p$, and an output $y$, and "score" it (higher is better). The main useful property of scoring rules is that they should be \emph{proper}. This means that, letting $S(p, q) \equiv E_{y \sim q}[S(p, y)]$, we should have $S(q,q) \geq S(p, q)$ for all $p$. There are nice characterizations of scoring rules via convex functions.

In our case each agent is implicitly reporting a distribution when they give their ad: providing ad $z_i$ leads to output distribution $p(y|x, z_i)$ from the LLM. Suppose the LLM outputs tokens according to a different distribution $p'$. Using the scoring rule as a measure of the "quality" of the tokens/sequences from this output distribution, we'd have $E_{y \sim p'}[S(p(\cdot|x, z_i), y)] = S(p(\cdot|x, z_i), p')$ as the expected score. This is minimized (in the second argument) at $p(\cdot|x, z_i)$ if the scoring rule is proper.

My (still vague) idea is that the allocation function should have the structure of a scoring rule: if ad $i$ wins the auction, then the output should be what maximizes the expectation of $S(p,y)$ for that agent, namely the output distribution $p(y|x, z_i)$.
}

\sscomment{Overloaded definition for $S$. This is kind of implementation of relevance oracle or relevance-based valuation for advertiser's true valuation. This means that even for single allocation, even if bidder $i$ is not selected, $i$ realizes positive utility.}


% We further define several notations to introduce the seminal result by~\cite{}
According to the seminal result by~\cite{myerson1981optimal}, there exists a unique payment rule to implement any monotone allocation function, where monotonicity and implementability of an allocation function is formally defined as follows.
% To this end, we first need to define the definition of implementable allocation rule along with several other notations.


% \begin{definition}[DSIC]
%     A mechanism $\Mec = (\x, \b)$ is dominant-strategy incentive-compatible (DSIC) if truthful bidding is a dominant strategy for every advertiser $a \in \cA$.
% \end{definition}

% Our main objective is to characterize DSIC mechanism with desirable allocation rule, to meet the user satisfaction as well as the advertiser's utility and the platform's revenue.

\begin{definition}[Monotonicity/Implementation]
    An allocation rule $\x$ is monotone if the function $x_i(z ; b_{-i})$ given $b_{-i}$ is nondecreasing in $z$.
    Further, $\x$ is implementable if there exists a corresponding payment rule $\p$ such that $\Mec = (\x, \p)$ is DSIC.
\end{definition}

% The seminal result by~\cite{myerson1981optimal}


% \begin{definition}[Implementation]
    
% \end{definition}

Finally, Myerson's lemma can be written as follows.
\begin{lemma}[\cite{myerson1981optimal}]\label{lem:myerson}
    Consider a single-parameter auction environment.
    \begin{enumerate}
        \item An allocation rule $\x$ is implementable if and only if it is monotone.
        \item If $\x$ is monotone, then there exists a unique payment rule $\p$ such that $\Mec = (\x, \p)$ is DSIC assuming that $p_i(\b) = 0$.
        \item The payment rule is given by
        \begin{align}
            p_i(\q, b_i, \b_{-i}) = \int_{0}^{b_i} z \cdot \frac{d}{dz} x_i(\q, z, \b_{-i}) dz \, .\label{eq:myerson-pay}
        \end{align}
    \end{enumerate}
\end{lemma}

We further require the mechanism to satisfy the participation constraint so that the advertisers are incentivized to join the mechanism given the outside option of utility zero.
\begin{definition}[Individual rationality]
    A mechanism $\Mec$ is individually rational (IR) if
    \begin{align*}
        u_i(\q, \b) \ge 0,
    \end{align*}
    for any $\q, \b$ and any $i \in \A$.
\end{definition}





\paragraph{Social Welfare}
In the standard mechanism design, particularly from the conventional sponsored search auction's perspective, the social welfare is defined as the summation of the utility of every participants, formally,
\begin{align*}
    \SW = u_{\Mec}(\q, \b) + \sum_{i \in [n]}u_i(\q, \b) = \sum_{i \in [n]} v_i x_i(\q, \b).
\end{align*}

Importantly however, as discussed before, this does not well-capture the user satisfaction given the LLM's response.
Thus, our objective is not to maximize social welfare, but to maximize the following weighted version of the social welfare, which is often called as a \emph{quality variant} in the sponsored search auction, \eg see~\cite{aggarwal2009general} and~\cite{lahaie2007sponsored}.
\sscomment{Not quite sure if the current presentation is good.}
\begin{definition}[Quality variant social welfare]
    A mechanism's quality variant social welfare is
    \begin{align*}
        \QSW = \sum_{i \in [n]}q_iv_i \cdot x_i(\q, \b).
    \end{align*}
\end{definition}

Let's take a break, and verify whether our problem setup and objective thus far makes sense with the following two toy examples. 
\begin{example}
    Consider two advertisers with bids $b_1 = 10-\eps$ and $b_2 = 1$.
    Suppose that given a certain query $x$, the relevance are computed to be $q_1 = 0.1$ and $q_2 = 1$.
    That is, $a_1$ is very irrelevant to the query $x$ whereas $a_2$ is highly related.
    Our choice of allocative efficiency selects ad $a_2$ since $1 \cdot 1 > (10-\eps) \cdot 0.1$, which is reasonable since $a_1$ is too much irrelevant to the query, thereby having a large change of ruining the user experience. 
    Also, the corresponding payment by Lemma~\ref{lem:myerson} will be the second price $1-0.1\cdot \eps \approx 1$, which would be also reasonable to advertiser $2$.
\end{example}
\begin{example}\label{ex:large-price}
    On the other hand, consider a scenario where $b_1 = 10+\eps$.
    In this case, allocative efficient mechanism selects $a_1$, and the corresponding payment will be minimal $z$ satisfying $z \cdot q_1 = 0.1 \cdot z> b_2q_2 = 1$, which is $10$.
    Would this make sense to the advertiser $1$?
    Yes, under our assumption that ``agent's true valuation is $v_1 = b_1$ regardless of the query and output''.
    But given that the relevance is \emph{significantly} small, the impact of the advertisement will be also desperate.
    In short, advertiser $1$ would have not written $b_1 = 10 + \eps$ for such query.
\end{example}

\sscomment{One way of presentation is to start with $q_ib_i$, which might be cleaner from modeling perspective, but current way might be able to more emphasize our motivation.}
The above examples hints that we may need to adjust our assumption such that \emph{agent realizes the same valuation regardless of the context}.
Thus, we consider a slightly different stylized model as follows.
\begin{definition}[Relevance-based valuation]\label{def:rel-value}
    Given a query $x$ and the corresponding relevance $q_i = r(a_i | x)$, the advertiser $i$'s true valuation of advertising $a_i$ is $\tv_i = q_i \cdot v_i$.\footnote{Ideally, one may ask advertiser to write very complicated multi-dimensional bids that may reflect advertiser's preference as a function of every possible $x$ and $y_i$, but this is obviously impractical from the advertiser's perspective.
    Moreover, this assumes that the set of advertisers $\cA$ is static, which is not practical too.
    Thus, our stylized model can be thought of an approximate version to mimic the ideal case in a practical manner, which is also similar to the philosophy of the autobidder that is pervasive in the modern online advertising, \eg~\cite{lucier2023autobidders}.\label{fn:1}} We also write $\tb_i = q_ib_i$ instead of $\tv_i$ when we deal with the bid instead of the valuation.
    \SLcomment{This is basically value/bid per impression rather than per click.}
\end{definition}
We denote this version of advertiser model as \emph{relevance-based valuation} setting, and the current version as a naive valuation setting.
\sscomment{This is analogous to the CTR - CPM transformation. How can we make different from standard SSA? To more relate to LLM? Introduce user utility}
\SLcomment{Two vague ideas to relate it more to LLMs:
\begin{enumerate}
    \item Understand what objective RAG allocation is optimizing for, and perhaps user utility comes into play there. Intuitively, we could say that if all bids are the same then the LLM output defaults to the usual RAG formula that only cares about relevance of docs (and not bids), and this is best for user utility. As bids get different from each other and more weight gets put on a single advertiser, that advertiser's utility increases possibly at the expense of user utility.
    \item Second price computation for RAG output. Both the Renato and Aranyak papers assume that tokens are just generated probabilistically as output. But that's not the way LLMs are usually decoded in practice. See \url{https://towardsai.net/p/machine-learning/how-does-an-llm-generate-text} that Mohammad sent out. Decoding often involves a temperature setting, and that could change the allocation and second-price.
\end{enumerate}}
\sscomment{One question here: I think user might be better off by not using RAG with ad documents, but just responding the original output. Treating ad documents already discount user experience, \eg if all the ads are very irrelevant. Probably we still need an explicit user experiment function?}

\sscomment{For Definition 1.13, we can frame it as advertiser's value for click is $v_i$ and pCTR is $q_i$, so the relevance oracle essentially predicts the CTR. Alternatively we can also define another oracle for such pCTR. Then this will be more consistent with Aranyak's paper (still we have different features like ex-post IC, exogenous prominence, etc).}


Then, the social welfare can be rewritten as
\begin{align*}
    \SW = \sum_{i \in [n]}\tv_i \cdot x_i(\q, \b) 
 =\sum_{i \in [n]}q_iv_i \cdot x_i(\q, \b) ,
\end{align*}
which in fact coincides with the quality variant in the naive valuation setting.


However, as discussed above, user experience is much more important for LLM advertising, since the user only reads the ad-incorporated output directly, unlike the traditional sponsored search auction in which the user can see one or two slots of sponsored ads preceded by the search engine result contents.

\sscomment{We can motivate it via user satisfaction vs ctr as per position paper.}
Thus, we explicitly consider the \emph{user's utility} for social welfare as well, where
\begin{align*}
    u_{\User} = \sum_{i \in [n]}f(q_i)x_i,
\end{align*}
where $f(q_i)$ captures the user's utility when $a_i$ is selected and incorporated in the output.
Then, the social welfare can be rewritten as
\begin{align}
    \SW = \sum_{i \in [n]}(\tv_i  + f(q_i))\cdot x_i(\q, \b) ,\label{eq:final-sw}
\end{align}
where $f: \R^n \to \R$ is a function that represents the user's utility.





Social welfare well-balances the trade-off between the user experience, platform revenue, and advertiser utility. 
On the other hand, it does not capture the \emph{fairness among the advertisers}, since it selects a single ad in a deterministic manner.
In this context,  we also consider the following well-known Nash social welfare.
\sscomment{not sure if it's fine to let it be NSW. This is not multiplication of the individual payoff (since we don't account for the utility loss from the payment for each advertiser).}
\begin{definition}[Nash social welfare]
    A mechanism's Nash social welfare is defined as
    \begin{align}
        \NSW = \prod_{i \in [n]}  x_i(\q, \b)^{\tv_i + f(q_i)}.\label{eq:nsw}
    \end{align}
    % If a mechanism (allocation rule) maximizes NSW, then the mechanism is said to have the maximal Nash social welfare (MNW).
\end{definition}
Note that it is consistent with the~\eqref{eq:final-sw} in the sense that if one takes logarithm at~\eqref{eq:nsw}, then it becomes
\begin{align}
    \sum_{i \in [n]}(\tilde{v}_i + f(q_i)) \log x_i,
\end{align}
which simply replaces $x_i$ by $\log x_i$ from~\eqref{eq:final-sw}.
Intuitively, if mechanism sets $x_i = 0$ for some $i \in [n]$, then $\NSW$ becomes zero, implying that the mechanism should guarantee some nonnegative probability of selection to every ads.
Indeed, it is well known from the literature, that maximizing the Nash social welfare is equivalent to the proportional fair allocation, see~\cite{kelly1998rate,lan2010axiomatic,yang2007vcg}, and also the competitive equilibrium from equal incomes (CEEI) by~\cite{arrow1981handbook,caragiannis2019unreasonable}. \sscomment{We discuss more details in the appendix.}



\sscomment{Probably we can discuss revenue maximization using virtual valuation and ironing for Bayesian mechanism in the appendix, but would it be worth?}


We often consider the following two instantiation of the user utility function.
\begin{definition}[Thresholded rule]\label{def:single-thres}
    \emph{Thresholded rule} is given by $f(q_i) = (-\infty)\cdot \Ind{q_i < \tau}$ for some threshold $\tau \ge 0$.
    That is, the mechanism will not consider any $a_i$ whose relevance is strictly smaller than the specified threshold $\tau$.
\end{definition}
This approach would eventually filters some irrelevant ads in advance, which can be commonly seen in the standard search advertising, \eg ~\cite{hillard2010improving} and~\cite{aiello2016role}.

\begin{definition}[Linear rule]
    \emph{Linear rule} is defined as $f(q_i) = \theta \cdot q_i$ for some $\theta \ge 0$.
    That is, the user's utility is proportional to how much the ad is related to the query.
\end{definition}


% \footnote{This is not the case for the standard sponsored search auction. This is because once the ad slot is determined in the search engine results page (SERP), the decrement of the }




% \sscomment{Todo: do not mention below. But instead of maximizing social welfare, say that we are interested in  allocative efficiency as per Sebastien's paper. Then, further, we can discuss that allocative efficiency can be viewed as a scenario where each advertiser's utility is actually $v_i \cdot q_i$ and then maximizing social welfare. Discuss that the resulting mechanism would be the same. 
% We can also mention that alternatively, one may view this as accounting for the user's utility as $u_{user} = q_i = r(a_i | x)$. Then, we are actually maximizing log linear social welfare, \ie $\sum log u_i$, which is maximizing $q_i \cdot b_i$.
% }
% Importantly, however, as discussed in the relevance oracle and correspondingly in Discussion~\ref{dc:relevance-ctr}, the advertiser would realize different utility based on how the induced output response is relevant to its ad.
% Thus, we consider an adjusted version of advertiser's utility as follows.
% \begin{align}
%     u_i(\q, \b) = v_i q_i \cdot x_i(\q, \b) - p_i(\q, \b), \label{eq:util-adjusted}
% \end{align}
% \ie the valuation is weighted by the relevance score $q_i = r(a_i | x)$.
% We simply write \emph{utility} to denote ~\eqref{eq:util-adjusted}.
% In fact, an acute reader may have noticed, this is equivalent to assuming that the advertiser $i$'s true valuation for being advertised given the query $x$ is $v_i q_i = v_i r(a_i | x)$.
% \sscomment{Also mention that this is similar to the quality variant in Google's sponsored search auction, see \href{https://en.wikipedia.org/wiki/Sponsored_search_auction}{link}, \href{https://web.stanford.edu/~saberi/sponsored-search.pdf}{link2} and also this is studied in~\cite{aggarwal2009general}.}


\paragraph{Computational Efficiency}
To operate certain mechanisms in the real world, 
% The design of optimal mechanism is appealing, however, 
it is necessary to consider the practicality of the mechanism in terms of its running time, \eg see~\cite{hartline2009simple}.
This is even more critical for online ad auction as display ad or search ad typically requires the total latency of no more than $100$ms, \eg see~\cite{wang2017display} and~\cite{yuan2013real}.
We formally define several notions of complexities to characterize the mechanism's efficiency.

We formally define the complexity given the abstraction of the LLM and the similarity module.
\begin{definition}[Query complexity]
    % The mechanism has access to the following oracles: (1) \emph{Similarity oracle} computes the relevance of the ad $a$ to the query $x$, and (2) \emph{LLM oracle} computes the output $y$ given the query $x$, selected ad $a$.
    % Then, t
    The \emph{query complexity} for the relevance/LLM oracle for a mechanism is defined by the number of times required to call the oracle to run a mechanism, respectively.
\end{definition}

Aside from query complexity, our mechanism should be also computationally feasible to compute the payment function and allocation function in a similar vein to~\cite{hartline2009simple}.
We are basically interested in the overall \emph{time complexity} to run a specific mechanism assuming that LLM and similarity query only requires a constant time, and the \emph{query complexity} itself since LLM query, for instance, can be highly expensive.

In short, our objective is to design a mechanism that has (i) less query complexity to reduce the cost of running the LLM and the similarity module, (ii) less time complexity to minimize the overall running time, and finally (iii) more efficiency in terms of various desiderata, \eg the platform's revenue or social welfare.


Finally, given the user utility function $f(\cdot)$, we say that a mechanism is EPIC if it satisfies DSIC, IR, and maximizes social welfare, and FAIR if it satisfies DSIC, IR, and maximizes Nash social welfare.

% \begin{enumerate}
%     \item Mechanism collects bids $\b = (b_1,b_2,\ldots, b_n)$ from the advertisers.
%     \item Mechanism computes the relevance $\q = (q_1,q_2,\ldots, q_n)$ from relevance oracle.
%     \item Mechanism determines the allocation $\x(\b, \q) \in \R^n$ such that $||\x||_1 \le 1$, and the payment function $\p(\b, \q) \in \R^n$.\footnote{The }
%     \item LLM oracle constructs the final output $y_i = l(a_i, x)$ given that $a_i$ is selected above.
% \end{enumerate}
% Note that $x_i$





\section{Single Allocation Mechanism}
\subsection{EPIC mechanism}


To obtain the EPIC mechanism, it is necessary to first derive the allocation rule that maximizes $\SW$.
In case the user utility function $f(\cdot)$ is finite for any value, one can simply compute
\begin{align*}
    \argmax_{i \in [n]} \tilde{b}_j + f(q_j),
\end{align*}
and apply the Myerson's lemma~\ref{lem:myerson}.
However, one needs to be careful if $f(\cdot)$ is not finite, \eg the thresholded rule.

In what follows, we explicitly derive the allocation and payment function for the thresholded rule and linear rule.
Note that any other general function $f(\cdot)$ can be dealt similarly.

\paragraph{Thresholded rule}
We start with our first result stating the existence and uniqueness of EPIC mechanism for the thresholded rule.
\begin{theorem}\label{thm:single-epic}
    Consider the thresholded rule $ f(q_i) = (-\infty)\cdot \Ind{q_i < \tau}$ for some $\tau \ge 0$.
    Given a query $x$, let $\cA(x) = \{i \in [n]: q_i \ge \tau\}$.
    Then, the following mechanism is the unique EPIC mechanism
    \begin{align}
        \Mec  = \begin{cases}
                        (x_i, p_i) &= (1, \max_{j \in \cA(x) \setminus \{i\}} q_j b_j) \,\, \mbox{if $i = \argmax_{j \in \cA(x)} q_j b_j$ and $i \in \cA(x)$}
                        \\
                        (x_i, p_i) &= (0,0) \,\, \mbox{otherwise}
                        \end{cases}
                        \label{eq:single-epic}
    \end{align}
\end{theorem}


\begin{proof}
    If $\cA(x) = \emptyset$, then $x_i = 0$ for every $i \in [n]$ and the proof folows.
    Suppose $|\cA(x)| \ge 1$.
    If any $i$ such that $i \notin \cA(x)$ has $x_i = 1$, then the social welfare becomes $-\infty$, which is strictly worse than allocating nothing, \ie $x_i =0$ for any $i \in [n]$.
    So $x_i > 0$ only if $i \in \cA(x)$.
    Thus we restrict our attention to the set $\cA(x)$ instead of $\cA$.

    Then, given that $|\cA(x)| \ge 1$, it is straightforward to see that the allocation rule defined in~\eqref{eq:single-epic} maximizes the social welfare.
    
    To obtain the payment function, we apply Lemma~\ref{lem:myerson} to the allocation function above.
    Notice that we set $z$ as a proxy for $\tb_i = q_i b_i$, and integrate over $z$, \ie
    \begin{align}
            p_i(\q, b_i, \b_{-i}) 
            &= \int_{0}^{\tb_i} z \cdot \frac{d}{dz} x_i(\q, z, \b_{-i}) dz
            \nonumber
            \\
            &=
            \max_{j \in \cA(x) \setminus \{i\}} q_j b_j.\label{eq:single-pay}
        \end{align}
    % Since the allocation is deterministic, $x_i(\q, z, \b_{-i})$ is always zero if $z < \max_{i\neq j \in \cA} q_jb_j$, and $1$ otherwise.
    % Therefore, the resulting payment function is
    % \begin{align}
    %     p_i(\q, b_i, \b_{-i}) = \frac{\max_{i \neq j \in \cA} q_j b_j}{q_i}.\label{eq:single-pay}
    % \end{align}
    Finally, such a mechanism is individually rational.
    This is because if $i \notin \cA(x)$, then $u_i(\q, \b) = 0$.
    Else, if $i = \argmax_{j \in \cA(x)} q_j b_j$, then  $u_i(\q, \b) = q_iv_i - \max_{j \in \cA(x)\setminus \{i\}} q_j b_j \ge 0$, and $u_i(\q, \b) = 0$ otherwise.
    Since the allocation function $\x$ is the only allocation function that maximizes the social welfare and Myerson's lemma implies the uniqueness of the payment function to implement such allocation function, $\Mec$ is the only EPIC mechanism given the thresholded rule.
\end{proof}


\begin{discussion}
    One may wonder if the truthfulness of the mechanism in Theorem~\ref{thm:single-epic} implicitly assumes that the advertisers know the similarity $q_i$ (or others $q_{-i}$) in advance, but this is not true.
    Indeed, notice that the payment function in~\eqref{eq:single-pay} is entirely determined by the second largest $b_a q_a$, so any advertiser cannot affect his/her utility by deviating from truthful report.
\end{discussion}

% \begin{discussion}
%     We emphasize that the resulting payment function is \emph{different} from the ones in the quality variant of the sponsored search auction by~\cite{aggarwal2009general} and~\cite{lahaie2007sponsored}, as described in Example~\ref{ex:large-price}.
%     Indeed, if we consider the allocative efficiency in the naive valuation setting, the corresponding payment will be $\max_{j \in [n] \setminus \{i\}} q_j b_j / q_i$ for selected $a_i$, which is much larger than~\eqref{eq:single-pay}.
% \end{discussion}

% The simplest approach is to deterministically decide the winner to be the one that maximize $q_i b_i$, \ie $x_a(\q, \b) = 1$ iff $a = \argmax_{a \in \cA} q_a b_a$ and $0$ otherwise.
% To implement such an allocation rule in a truthful manner, 




% In this case, according to Myerson's lemma~\ref{lem:myerson}, the resulting payment rule will be to charge the winner the second price.
% Precisely,
% \begin{align*}
%     p_a(q_i, b_i, \q_{-i}, \b_{-i}) = z \quad \text{s.t.} \, \max b_i q_i \le z q_a \, .
% \end{align*}
% Therefore, we obtain
% \begin{align}
%     p_a(q_i, b_i, \q_{-i}, \b_{-i}) = \frac{\max_{a \neq i \in \cA} q_i b_i}{q_a}.\label{eq:single-pay}
% \end{align}

% \begin{theorem}\label{thm:single-deter-dsic}
%     Consider RAG-based LLM advertising auction with bids $\b$.
%     The following mechanism $\Mec$ with uniform tie breaking rule is DSIC:
%     \begin{align}
%         \Mec  = \begin{cases}
%                         (x_a, p_a) &= (1, \max_{a \neq i \in \cA} q_i b_i/q_a) \,\, \mbox{if $a = \argmax_{a \in \cA} q_a b_a$}
%                         \\
%                         (x_a, p_a) &= (0,0) \,\, \mbox{otherwise}
%                         \end{cases}
%                         % \label{eq:single-deter-mec}
%     \end{align}
% \end{theorem}
% \begin{proof}
%     \sscomment{Directly follows from Myerson, but expand}
% \end{proof}

The following theorem further characterizes the query and time complexity to run such mechanism.
\begin{theorem}\label{thm:single-epic-comp}
    The mechanism defined by~\eqref{eq:single-epic} has LLM query complexity of $O(1)$, relevance query complexity of $O(n)$, and time complexity of $O(n)$.
    % \begin{itemize}
    %     \item LLM query complexity of $O(1)$.
    %     \item 
    %     \item Time complexity of $O(\log n)$.
    % \end{itemize}
\end{theorem}
\begin{proof}
    To execute the mechanism, it first needs to compute the relevance measure $q_i = r(x | a_i)$ for each $i \in [n]$, which requires $n$ calls of relevance oracle.
    Given that we obtained $\q$, collected $\b$, the mechanism only needs to calculate $b_a q_a$ for each $a$ which requires $O(1)$ time complexity.
    Then, it needs to compute the  $i = \argmax_{j \in \cA(x)} b_jq_j$ and the second largest $\argmax_{j \in \cA(x) \setminus \{i\}}q_jb_j$, which requires $O(n)$ by going over the entire list once and store the maximal and second maximal index.
    Subsequently, given the maximal and second maximal index, the payment function simply computes~\eqref{eq:single-pay} in $O(1)$ time.
    Thus, the overall time complexity of the mechanism is $O(n)$
    Given that the mechanism selected $a_i$, we simply call the LLM oracle once to obtain the output $y = l(a_i,x)$.
\end{proof}


\paragraph{Linear rule}
The EPIC mechanism for the linear rule can be similarly obtained.
\begin{theorem}\label{thm:single-epic-linear}
    Consider the linear rule $ f(q_i) = \theta \cdot q_i$ for some $\theta \ge 0$.
    Then, the following mechanism is the unique EPIC mechanism
    \begin{align}
        \Mec  = \begin{cases}
                        (x_i, p_i) &= (1, \left ( (\max_{j \in \cA \setminus \{i\}} q_j (b_j + \theta) - q_i\theta\right)^+ \,\, \mbox{if $i = \argmax_{j \in \cA} q_j (b_j + \theta)$}
                        \\
                        (x_i, p_i) &= (0,0) \,\, \mbox{otherwise}
                        \end{cases}
                        \label{eq:single-epic-linear}
    \end{align}
\end{theorem}
\begin{proof}
    similar.
\end{proof}

\begin{discussion}
    \sscomment{Discuss that it would be better to not advertise in case payment is zero due to small $q_j(b_j + \theta)$.}
\end{discussion}

% \begin{discussion}\label{dc:welfare}
    
    % Notice that the allocation function completely determines the social welfare of the system, \ie the summation of the utility of every participants, since the monetary transfer is cancelled out between the players.\footnote{In fact, as per the revenue equivalence theorem by~\cite{myerson1981optimal}, the revenue of the mechanism designer for any DSIC mechanism is equivalence if the allocation function is the same.}
    % Thus, one main question is whether there exists a mechanism that implements a specific allocation function, where the definition of the implementation is as follows.
% \end{discussion}

\subsection{FAIR mechanism}

The following theorem explicitly characterizes the FAIR mechanism.
\sscomment{Further discuss the importance of having a randomized output from the LLM perspective. \Eg, diversity, text degeneration (refer \href{https://arxiv.org/pdf/1904.09751.pdf}{The Curious Case of Neural Text Degeneration
}), etc.}

\begin{theorem}\label{thm:single-fair}
    Consider the thresholded rule $ f(q_i) = (-\infty)\cdot \Ind{q_i < \tau}$ for some $\tau \ge 0$.
    Given a query $x$, let $\cA(x) = \{i \in [n]: q_i \ge \tau\}$.
    Then, the following mechanism is the unique FAIR mechanism: for any $i \in \cA(x)$,
    \begin{align}
        \Mec = (\x,\p) = \begin{cases}
            x_i= \frac{\tb_i}{w_i+ \tb_i}
            \\
            p_i= w_i \parans{\frac{w_i}{w_i + \tb_i} - 1 - \ln \frac{w_i}{w_i+ \tb_i}}
        \end{cases}
        % \Mec = (x_i,p_i)_{i \in [n]} = \left( \frac{q_i b_i}{\sum_{j \in [n]} q_j b_j}, \frac{w}{q_i} \parans{\frac{w}{w + q_ib_i} - 1 - \ln \frac{w}{w+ q_ib_i}} \right)_{i \in [n]} \, .
        \label{eq:single-fair-mec}
    \end{align}
    where $w_i = \sum_{j \in\cA(x) \setminus \{i\}} \tb_j$, and for $i \notin \cA(x)$, then $x_i = p_i = 0$.
\end{theorem}
\begin{proof}
    Similar to the proof of Theorem~\ref{thm:single-epic}, we can focus our attention to the set $\cA(x)$ instead of $\cA$, \ie for $i \notin \cA(x)$, we necessarily have $p_i = x_i = 0$.
    Note that if $\cA(x) = \emptyset$, then we are done.
    Suppose not.
    First, to compute an allocation that maximizes NSW, recall that we should maximize
    \begin{align*}
        \NSW = \prod_{i \in \cA(x)} x_i^{\tb_i},
    \end{align*}
    such that $\sum_{i \in \cA(x)} x_i = 1$ and $x_i \ge 0$ for any $i \in \cA(x)$.
    Set up the Lagrange function $L$ as follows.
    \begin{align*}
        L(\x, \lambda) = \prod_{i \in \cA(x)} x_i^{\tb_i} + \lambda(-1 + \sum_{i \in \cA(x)}x_i ).
    \end{align*}
    By taking the partial derivative with respect to $x_i$ for $i \in [n]$ and $\lambda$, we obtain a system of equations
    \begin{align*}
        \frac{\partial L}{\partial x_i} &= \tb_i \prod_{i \in \cA(x)} x_i^{\tb_i} / x_i + \lambda = 0, \forall i \in \cA(x)
        \\
        \frac{\partial L}{\partial \lambda} &= -1 + \sum_{i \in \cA(x)}x_i = 0 .
    \end{align*}
    To solve for $\x$, we first obtain
    \begin{align*}
        \tb_i \prod_{i \in \cA(x)} x_i^{\tb_i} / x_i = C,
    \end{align*}
    for some constant $C$ for any $i \in \cA(x)$.
    This yields proportional relationship of
    \begin{align*}
        \frac{\tb_i}{x_i} = c,
    \end{align*}
    for some constant $c$ for any $i \in \cA(x)$.
    Plugging into $\sum_{i \in \cA(x)} x_i =1$ yields the desired allocation.
    
    
    Now, our payment rule can be computed as
    \begin{align*}
        p_i(\q, \b) = \int_{0}^{\tb_i} z \cdot \frac{d}{dz}\left(\frac{z}{\sum_{j \in \cA(x)} q_j b_j}\right) dz \, .
    \end{align*}
    Write $w_i = \sum_{j \in \cA(x) \setminus \{i\}} \tb_j$.
    Computing the integral above, we obtain
    \begin{align}
        p_i(\q, \b)
        &= \int_{0}^{\tb_i} z \cdot \frac{d}{dz}\left(\frac{z}{w_i + z}\right) dz \nonumber
        \\
        &= \int_{0}^{\tb_i} z \cdot \left(\frac{w_i}{(w_i + z)^2}\right) dz \nonumber
        \\
        &= \int_{0}^{\tb_i} \frac{w_i z}{(w_i +  z)^2} dz \nonumber
        \\
        &= w_i\left(\frac{w_i}{z + w_i} + \ln {(z + w_i)}\right) \Big|_0^{\tb_i}\nonumber
        \\
        &= 
        w_i \parans{\frac{w_i}{w_i + \tb_i} - 1 - \ln \frac{w_i}{w_i + \tb_i}} \, .
    \end{align}
    Finally, such a mechanism is individually rational since for $i \notin \cA(x)$ it is trivially zero and for $i \in \cA(x)$, we have
    \begin{align*}
        u_i(\q, \b) &= \tb_i \frac{\tb_i}{w_i + \tb_i} - w_i \parans{\frac{w_i}{w_i + \tb_i} - 1 - \ln \frac{w_i}{w_i+ \tb_i}}
        \\
        &=
        b_i + w_i \ln \frac{w_i}{w_i + \tb_i}
        \\
        &\ge
        b_i - w_i \cdot \frac{b_i}{w_i} \ge 0,
    \end{align*}
    where in the first inequality we use $\ln(1 + t) \le t$ for $t > -1$.
    
    Since the provided allocation function $\x$ is the only allocation function that maximizes NSW,  Myerson's lemma implies the uniqueness of the payment function to implement such allocation function, $\Mec$ is the only FAIR mechanism.
\end{proof}
\sscomment{A picture for it, and probably discuss some points? (convexity, etc)}

\begin{discussion}
    We note that the mechanism~\eqref{eq:single-fair-mec} can be implemented as a randomized mechanism that selects an ad based on the probability $\x$.
    Also, the utility can the corresponding payment can be thought of as an expected utility and expected payment, and all the arguments still hold.
    This is essentially because we assume linear utility of $u_i = \tv_i x_i - p_i$, \ie due to the linearity of the expectation.
    For instance, if we assume risk-averse advertiser with quasi linear utility, \eg $u_i= \phi(\tv_i x_i) - p_i$ for some nonlinear function $\phi$, then our randomized mechanism may not simply imply the shown properties above.
\end{discussion}

\begin{theorem}
    The mechanism defined by~\eqref{eq:single-fair-mec} has LLM query complexity of $O(1)$, relevance query complexity of $O(n)$, and time complexity of $O(n)$.
\end{theorem}
\begin{proof}
    The only difference from Theorem~\ref{thm:single-epic-comp} for the EPIC mechanism is that it needs to random sample the outcome based on the desired allocation rule $\x$ which requires $O(n)$ time complexity, \eg sampling a random number given a corresponding interval for each $i \in [n]$.
    This does not change any time/query complexity.
\end{proof}


\begin{theorem}\label{thm:single-fair}
    Consider the linear rule $ f(q_i) = \theta q_i$ for some $\theta \ge 0$.
    Then, the following mechanism is the unique FAIR mechanism: for any $i \in \cA$,
    \begin{align}
        \Mec = (\x,\p) = \begin{cases}
            x_i= \frac{\tb_i + f(q_i)}{w'_i+ \tb_i+f(q_i)}
            \\
            p_i= w'_i \parans{\frac{w'_i}{w'_i + \tb_i+f(q_i)} - 1 - \ln \frac{w'_i}{w'_i+ \tb_i + f(q_i)}}
        \end{cases}
        % \Mec = (x_i,p_i)_{i \in [n]} = \left( \frac{q_i b_i}{\sum_{j \in [n]} q_j b_j}, \frac{w}{q_i} \parans{\frac{w}{w + q_ib_i} - 1 - \ln \frac{w}{w+ q_ib_i}} \right)_{i \in [n]} \, .
        \label{eq:single-fair-mec}
    \end{align}
    where $w'_i = \sum_{j \in\cA \setminus \{i\}} \left(\tb_j+f(q_j) \right)$.
\end{theorem}
\begin{proof}
    \sscomment{TBD. Actually payment should be checked carefully.}
\end{proof}


\subsection{Further Discussions}\label{sec:single-further-disc}
To operate our LLM ad auction in practice, it is important to implement the relevance and LLM oracle as well as choose a suitable function $f(\cdot)$ to maintain the output quality.

\sscomment{Mention that we compare these things in the experiments}

\paragraph{Choice of relevance measure: efficiency vs complexity}
Our relevance oracle only retrieve the parameters $a_i$ and $x$ as the input.
However, more precise measure to estimate the relevance between an ad and the user experience might be to include the eventual output $y_i$ in the input as well, \ie
\begin{align*}
    q_i = r(a_i | y_i, x).
\end{align*}
We denote this version of relevance oracle by \emph{output-dependent} relevance oracle.
\sscomment{Keivan: discuss how it can be implemented using LLM distribution?}
Given the redefined notion of relevance oracle, the characterization of the proposed mechanism in Theorem~\ref{thm:single-epic} and~\ref{thm:single-fair} remain the same.
\SLcomment{I don't see how this mechanism would work. To compute the output $y$ the mechanism needs to have the relevance scores. But here the relevance scores depend on the output $y$. I don't see how to make that circularity work.}
\sscomment{It works as follows: for every $i$, it precomputes $y_i$, \ie the outputs. Then, we can compute the relevance. Then, we run the auction and it outputs which $y_i$ to take among $i \in [n]$. We can elaborate on that.}
The computational complexity, however, changes since the relevance oracle itself requires the information on $y_i$.
The following theorem
\begin{theorem}
    Given a output-dependent relevance oracle, the mechanism defined by~\eqref{eq:single-epic} and~\eqref{eq:single-fair-mec} requires LLM query complexity of $O(n)$, relevance query complexity of $O(n)$, and time complexity of $O(n)$.
\end{theorem}
\begin{proof}
    The only difference is that the single call of relevance oracle requires that it already knows $y_i$, \ie we have to call LLM oracle for every $i \in [n]$ to determine the outcome of the mechainsm.
    Thus, only the LLM query complexity is changed to be $O(n)$.
\end{proof}

Alternatively, one might also consider $q_i = r(a_i | y_i)$ as the relevance measure regardless of the original query.
Such a choice would not affect the query complexity and the mechanism.


\paragraph{Choice of the user utility $f(\cdot)$}
\sscomment{Choice of the user utility can be more various. Discuss them.}
% To prevent the user experience too bad in case all the available advertisements are not that relevant to the given query, one may screen out the set of advertisements whose relevance is not 

% \paragraph{Valuation model}
% \sscomment{Can also discuss the reasonableness of the valuation assumption $v_i q_i$ and what alternatives we may use.}

 

\section{Multiple Allocation Mechanism}
% In the standard sponsored search auction, given a user query, multiple ads can be advertised in a simultaneous manner if there are multiple slots for the advertisement.
% For instance, Google runs a variant of the generalized second price auction (CITE).
\sscomment{Our multi allocation mechanism is similar to position auction with dependent CTR - see \href{https://dl.acm.org/doi/pdf/10.1145/2668108}{survey}. Also section Auctions with Rich Bidding Language.}
So far, we focus on the setting in which the mechanism is only interested in advertising a single ad in the LLM's output.
In this section, we propose several approaches to advertise multiple ads at once given a single query.

Compared to the standard sponsored search auction with the explicit ad slots, it is not straightforward how one can adapt to advertise multiple ads at once for RAG-based LLM system due to the absence of the strict separation between the ads in the output.
Precisely, we are interested in the \emph{multiple allocation} (MA) mechanism that selects multiple ads and incorporates all of them in the response simultaneously.\footnote{We use \emph{single allocation} (SA) mechanism to denote the previous setting of single ad advertising.}
We often use $k$-MA to specify that $k$ ads are advertised at once, and $k$-MA setting to denote that we are interested in the class of $k$-MA mechanisms.
We will first discuss the output selection module given the set of ads to advertise, and then discuss the mechanism design problem of choosing the set.


To derive characterize desirable mechanisms, we first need to define the analogous notions of LLM and relevance oracles.
Let $\cA_k$ be the collection of every $k$-tuples which are subset of $\cA$, \ie $\cA_k = \{A: A \subset [n], |A| = k\}$.




\begin{definition}[LLM oracle]
    A LLM oracle $\ell(A, x)$ constructs the response $y_A$ consisting of a sequence of tokens that incorporates the set of ads $A \in \cA_k$ in the response to the query $x$.
\end{definition}

Suppose that we have defined the relevance oracle similar to Definition~\ref{def:rel-value}, \ie the relevance oracle gives us $q_A = r(A | x)$ for $A \in \cA_k$.
Then, we should define a proper notion of advertiser's true valuation on the output.
Formally, we need to model how an advertiser $i$ values the output $y_A$ if $i \in A$.
A naive approach would be to simply use $q_A v_i$, but this is not satisfactory as $q_A$ considers the relevance of the other ads in $A$.
Thus, since it is more likely that the induced output $y_A$ will be not only representing $i$ but also other ads $i \neq j \in A$, it is essential to capture the genuine relevance of $a_i$ against $y_A$.
Thus, we allow the relevance oracle to account for $y_A$ in the parameter similar to what is discussed in Section~\ref{sec:single-further-disc}.


\begin{definition}[Relevance oracle]
    A relevance oracle $r(a_i | x, y_A)$ computes a nonnegative real number $q_{A, i} \in [0,1]$ that represents the relevance of the ad $a_i$ given the query $x$ and corresponding output $y_A = \ell(A,x)$. \SLcomment{As before I'm worried that this is circular. We need the relevance to generate the output (at least in a RAG approach), but here the output depends on the relevance.} \sscomment{It would work similarly as discussed in Section~\ref{sec:single-further-disc}. Let me know if there's anything unclear. Also, I think this might be one point that makes our setup different from Aranyak's paper (from the multi allocation perspective). In their paper, they assume that their pCTR module computes average pCTR regardless of the actual output $y$, and assume that this is unbiased estimation over the expectation of generated output.
    This is to prevent the circular reasoning arisen there, but we don't suffer such circularity since the prominence are exogenously given once the set of ads are chosen.
    Note that they further consider incentive compatibility in an ex-ante manner given such averaging.}
\end{definition}

Then, we define the advertiser's private value as follows.
\begin{definition}[Relevance-based valuation]
    Under the $k$-allocation mechanism, each ad $a_i$ has a private value of $v_i \cdot q_{A,i}$ if the output is $y_A$ for $i \in A$ and $A \in \cA_k$.
\end{definition}
To develop the analogous notions of social welfare, we first need to define the user utility function.
Unlike from the SA mechanism, however, our definition of relevance oracle above only considers what the advertiser would realize as the relevance, since it considers the relevance of the single ad $a_i$ given $x$ and $y_A$.
The user's experience would be rather a function of $x, y_A$.
A reasonable benchmark of the quality of $y_A$ is how much it deviates from the original response $y$ which does not include any ad.
Note that this can be derived by computing the conditional probability in a token-by-token manner~\citep{vaswani2017attention, feizi2023online}, or measuring the semantic similarity between two output.
\sscomment{Discuss this more in the appendix. (implementation of distance oracle)} \SLcomment{This is interesting, what kind of concrete distance oracles have you considered so far?}
\sscomment{For the experiment, we simply use embedding distance between (i) $y_A$ and $x$ and (ii) $y_A$ and $y$. As discussed above, we can use the difference of the probability that LLM outputs. }

Thus, we introduce the following oracle.
\begin{definition}[Distance oracle]
    A distance oracle $d_A = d(y, y_A)$ computes a nonnegative real number $d_A \in [0,1]$ that represents the distance between the original output $y$ and the output $y_A$ which incorporates the set of ads $A$.
\end{definition}

\begin{discussion}
    \sscomment{Discuss that this in fact assumes that the original LLM's output is near optimal and very effective.} \SLcomment{This is a bit tricky given the different ways to do decoding, and the temperature parameter.}
\end{discussion}
\begin{discussion}
    \sscomment{Discuss that in fact, in the single allocation setting, we can use distance oracle to account for the user experience instead. This only requires $n$ further queries to the distance oracle, which is a bit more but not that much.}
\end{discussion}


Similar to the single allocation mechanism, we consider the following two representative rules for the user utility function.
\begin{enumerate}
    \item Thresholded rule: $f(d_A) = (-\infty) \cdot \Ind{d_A > \tau}$ for some $\tau \ge 0$.\footnote{Note here that the direction of the inequality is opposite from the relevance based thresholded rule in Definition~\ref{def:single-thres}.}
    \item Linear rule: $f(d_A) = \theta \cdot d_A$ for some $\theta \ge 0$.
\end{enumerate}
\sscomment{Notational issue - large distance means not good, so probably another notations is better (to make it analogous to the relevance)}



Then, the most general form of MA mechanism can be defined as follows.\footnote{In fact, the most general format would be ask each advertiser $i$ to write bid $b_{A,i}$ for every possible tuple $A \in \cA_k$, but this is practically impossible to implement as discussed in Footnote~\ref{fn:1}.}
\begin{definition}[$k$-allocation mechanism]
    Given the relevance and LLM oracle, a $k$-allocation mechanism $\Mec(\x, \p)$ that advertises $k$ ads at once can be completely characterized as follows.
    \begin{enumerate}
        \item Collect bids $\b = (b_1,\ldots, b_n) \in \R^n$ from the advertisers.
        \item Compute the relevance $\q = (q_A)_{A \in \cA_k} \in \R^{\binom{n}{k}}$ from the relevance oracle.
        \item Compute the distance $\d = (d_A)_{A \in \cA_k}$
        \item {\bf Allocation rule}: A set of ads $A \in \cA_k$ is selected according to the allocation function $\x(\q, \b) = (x_A)_{A \in \cA_k} \in \Delta_{\binom{n}{k}}$ where $\Delta_{\binom{n}{k}}$ denotes $\binom{n}{k}$-dimensional probability simplex.
        \item {\bf Payment rule}: Advertisers are charged based on the payment function $\p(\q, \b)\in \R^n$. We write $(p_{A,i})_{A \in \cA_k, i \in A}$ to denote what advertiser $i$ pays given that $A$ is selected.
        \item LLM oracle constructs the final output $y_{A^*} = l(A^*, x)$.
    \end{enumerate}
\end{definition}

Advertiser $i$'s utility can be written as follows.
\begin{align*}
    u_i = \sum_{A \in \cA_k: i \in A} \left( q_{A,i}x_A b_i - p_{A,i}\right) .
\end{align*}

The platform revenue is simply
\begin{align*}
    u_{\Mec} = \sum_{A \in \cA_k: i \in A}\sum_{i \in A} p_{A,i} .
\end{align*}
\sscomment{incorporate $x$}

The user utility can be written as
\begin{align}
    \sum_{A \in \cA_k}f(d_A)x_A.
\end{align}

Then, the social welfare for the $k$-allocation mechanism can be written as follows.
\begin{align}
    \SW &= \left( \sum_{i \in [n]} \sum_{A \in \cA_k: i \in A} q_{A,i} x_A \right) b_i + k\sum_{A \in \cA_k} f(d_A) x_A
    \\ &= \sum_{A \in \cA_k}\sum_{i \in A}( q_{A,i}b_i + f(d_A))x_{A}
\end{align}
where $f(d_A)$ denotes the user utility function given that the set of ads $A$ are selected.
\sscomment{It's a bit ambiguous how to define Nash social welfare. Given that we will not use ideal mechanism anyway, just skip it?}

\subsection{EPIC mechanism}
Similar to the single-allocation mechanism, we first present an EPIC mechanism. 


% Thus, we have the following general type of mechanism.

% \begin{enumerate}
%     \item Pick $A^* = \argmax_{A \in \cA_k} k\cdot f(d_A) + \sum_{i \in A}q_{A,i}b_i$.
%     \item Find $A' = \argmax_{A \in \cA_k^{-i}} k \cdot f(d_A) + \sum_{j \in A} q_{A,j}b_j$.
%     \item Charge each $i \in A^*$
%     \begin{align*}
%         p_{i} = \left( \sum_{j \in A'}  q_{A',j} b_j +  f(d_{A'}) \right)
%         - 
%         \left( \sum_{j \in A^* \setminus \{i\}}  q_{A,j} b_j +  f(d_{A^*}) \right)
%     \end{align*}
% \end{enumerate}

\begin{theorem}\label{thm:k-alloc-epic}
    Consider a $k$-allocation mechanism with the thresholded rule $f(d_A) = (-\infty) \cdot \Ind{d_A < \tau}$ for some $\tau \ge 0$.
    Then, the following mechanism is the unique EPIC mechanism:
    \sscomment{Use algorithm environment or Gray box.}
    \begin{enumerate}
        \item Filter out $A \in \cA_k$ such that $d_A < \tau$, and overwrite $\cA_k$ to be the set which excludes such $A$s. 
        \item Pick $A^* = \argmax_{A \in \cA_k} \sum_{i \in A}q_{A,i}b_i$.
        \item Find $A' = \argmax_{A \in \cA_k^{-i}} \sum_{j \in A} q_{A,j}b_j$, where $\cA_k^{-i} = \{A \in \cA: i \notin A, |A| =k\}$
        \item Charge each $i \in A^*$ the following:
        \begin{align*}
            p_{i} = 
            \sum_{j \in A'}  q_{A',j} b_j  
            - 
            \sum_{j \in A^* \setminus \{i\}}  q_{A,j} b_j 
        \end{align*}
    \end{enumerate}
\end{theorem}
\begin{proof}
    Given the thresholded rule, we can essentially redefine the set $\cA_k$ to be the one that excludes any $A \in \cA_k$ such that $d_A < \tau$.
    Then, it is straightforward to see that the allocation maximizing social welfare is given by
    \begin{align*}
        A^* = \argmax_{A \in \cA_k} \sum_{i \in A}q_{A,i}b_i.
    \end{align*}

    Note that this is obviously monotone over each bid.
    Thus, given the allocation above, for each $i \in A^*$, we calculate the Myerson pricing in what follows.
    
    For $i \in \cA$, we should compute the minimal bid $z$ that makes $i$ included in the winning package $A^* \in \cA_k$.
    To this end, let $A' \in \cA_k$ be the set satisfying the following:
    \begin{align*}
        A' = \argmax_{A \in \cA_k^{-i}} k \cdot f(d_A) + \sum_{j \in A} q_{A,j}b_j,
    \end{align*}
    where $\cA_k^{-i} = \{A \in \cA_k: i \notin A\}$.
    Thus, we will increase $z$ from zero to sufficiently large value such that there exists the first $A^* \in \cA_k$ with $i \in A^*$ satisfying
    \begin{align*}
        z + \sum_{j \in A^* \setminus \{i\}} q_{A^*,j}b_j \ge \sum_{j \in A'} q_{A',j}b_j.
    \end{align*}
    Therefore, given such $A^*$ and $A'$ as defined above, the payment to the advertiser $i$ will be
    \begin{align*}
        p_i = \sum_{j \in A'}  q_{A',j} b_j - \sum_{j \in A^* \setminus \{i\}} q_{A^*,j} b_j.
    \end{align*}

    Finally, to prove that the mechanism is individually rational, if $i \notin A^*$, then obviously $u_i \ge 0$.
    For $i \in A^*$, observe that
    \begin{align*}
        u_i &= q_{A^*, i} b_i - p_i
        \\
        &= \sum_{j \in A^*}q_{A^*, j}b_j - \sum_{j \in A'}q_{A', j}b_j  \ge 0,
    \end{align*}
    which finishes the proof.
\end{proof}


\begin{theorem}\label{thm:k-alloc-thres-complexity}
    The mechanism defined in Theorem~\ref{thm:k-alloc-epic} has LLM query complexity of $O(n^k)$, relevance query complexity of $O(n^k)$, and time complexity of $O(n^k)$.
\end{theorem}
\begin{proof}
    First, the mechanism starts with filtering out the undesired set of ads.
    Specifically, we first need to obtain the distance $d_A$ for every possible $A \in \cA_k$, which requires $\binom{n}{k} = O(n^k)$ queries to the distance oracle.
    Importantly, however, this assumes the knowledge on each $y_A$.
    Thus, this essentially requires $\binom{n}{k} = O(n^k)$ calls to the LLM oracle.
    
    Subsequently, we should compute the $\sum_{i \in A}q_{A,i} b_i$ for every nonfiltered $A \in \cA_k$.
    This requires at most $\binom{n}{k} = O(n^k)$ queries to the relevance oracle.
    Subsequently, to proceed step $2$, computing $\sum_{i \in A}q_{A,i} b_i$ requires $O(k \cdot \binom{n}{k})$ computation, and then selecting $A^*$ that maximizes this needs going through the entire list once, which is at most $\binom{n}{k} = O(n^k)$.
    
    Then, for each $i \in A^*$, we repeat the same process but without $i$.
    To this end, we can essentially reuse the $q_{A,i}$ obtained above, so there is no need of further queries to the relevance oracle.
    Also to select $A'$, we can reuse the quantities $\sum_{j \in A} q_{A,j} b_j$ computed above as well, thus the entire step $3$ requires $\binom{n-1}{k} = O(n^k)$ computation.
    
    Finally, the payment can be obtained via a single subtraction.
    Note that we don't need further query to the LLM oracle since we have computed all the $y_A$ in advance.
\end{proof}

\sscomment{We can possibly skip the following}
\begin{theorem}\label{thm:k-alloc-linear}
    Consider a $k$-allocation mechanism with the linear rule $f(d_A) = \theta \cdot d_A$ for some $\tau \ge 0$.
    Then, the following mechanism is the unique EPIC mechanism:
    \begin{enumerate}
        \item Pick $A^* = \argmax_{A \in \cA_k} k\cdot \theta d_A + \sum_{i \in A}q_{A,i}b_i$.
        \item Find $A' = \argmax_{A \in \cA_k^{-i}} k \cdot \theta d_A + \sum_{j \in A} q_{A,j}b_j$.
        \item Charge each $i \in A^*$
        \begin{align*}
            p_{i} = \left( \sum_{j \in A'}  q_{A',j} b_j + \theta d_{A'} \right)
            - 
            \left( \sum_{j \in A^* \setminus \{i\}}  q_{A,j} b_j +  \theta d_{A^*} \right)
        \end{align*}
    \end{enumerate}
\end{theorem}
\begin{proof}
    \sscomment{TBD. Follows from VCG but expands.}
\end{proof}

\begin{theorem}
    The mechanism defined in Theorem~\ref{thm:k-alloc-linear} has LLM query complexity of $O(n^k)$, relevance query complexity of $O(n^k)$, and time complexity of $O(n^k)$.
\end{theorem}
\begin{proof}
    \sscomment{Similar to Theorem 3.9 but expands a bit more.}
\end{proof}



\subsection{Simple and efficient mechanism}
\sscomment{Discuss that VCG is ideal and good, but is rarely used in practice. Refer \href{https://milgrom.people.stanford.edu/wp-content/uploads/2005/12/Lovely-but-Lonely-Vickrey-Auction-072404a.pdf}{Lovely but lonely Vickrey auction}.}

We here consider an efficient mechanism that requires less dependency on the oracles as well as less computational complexity.
From the advertiser's perspective, it is also desirable since the description of the mechanism is pretty intuitive and easy to understand.

\sscomment{Modified version to prevent negative payment and negative advertiser utility.}
\begin{definition}[Greedy mechanism with thresholded rule]\label{def:k-alloc-greedy}
    A greedy mechanism with thresholded rule for $k$-allocation setting proceeds as follows.
    \sscomment{Use algorithm environment or gray box.}
    \begin{enumerate}
        \item Parameter: $\tau \ge 0$. 
        \item Set $A = \emptyset$, $B = \emptyset$, $t=1$
        \item Initialize $\cA = [n]$.
        \item For each $i \in \cA$, let $A_i = A \cup \{i\}$.
        \item Compute $d_i = d(y_{A_i}, y)$ for each $i \in \cA$, and exclude $i$ from $\cA$ such that $d_i > \tau$.
        \item For each $i \in \cA$ and $j \in \cA_i$, compute $q_{A_i, j}$.
        \item For each remaining $i \in \cA$, compute
        \begin{align*}
            i_t = \argmax_{i \in \cA_k} \sum_{ j \in A_i} q_{A_i,j} b_j.
        \end{align*}
        % and compute
        % \begin{align*}
        %     i_s = \argmax_{i \in \cA_k^{-i_t}} \sum_{ j \in A_i} q_{A_i,j} b_j.
        % \end{align*}
        \item Update $A \gets A_{i_t}$ and $t \gets t+1$.
        \item Repeat step $3$ to $8$ until $t = k$.
        \item Given $A^* = \{i_1,\ldots, i_k\}$, sorts it so that $q_{A^*,i_1} b_{i_1} \ge a_{A^*,i_2} b_{i_2} \ge \ldots \ge q_{A^*,i_k} b_{i_k}$.
        \item For $t \in [k-1]$, $p_{i_t} = q_{A^*, i_t} b_{i_t} - q_{A^*, i_{t+1}} b_{i_{t+1}}$ and $p_{i_k} = q_{A^*, i_k} b_{i_k}$.
        % \item Compute $p_{i_t} =\sum_{j \in A_{i_s}} q_{A_{i_s},j} b_j -  \sum_{j \in A_{i_t} \setminus\{i_t\}} q_{A_{i_t},j} b_j $
        \item Return $A^* = \{i_1,i_2,\ldots, i_k\}$ and charge each $i_t$ the amount of $p_{i_t}$.
        
    \end{enumerate}
\end{definition}


% \begin{definition}[Greedy mechanism with thresholded rule]\label{def:k-alloc-greedy}
%     A greedy mechanism with thresholded rule for $k$-allocation setting proceeds as follows.
%     \sscomment{Use algorithm environment or gray box.}
%     \begin{enumerate}
%         \item Parameter: $\tau \ge 0$. 
%         \item Set $A = \emptyset$, $B = \emptyset$, $t=1$, and initialize $\cA = [n]$.
%         \item For each $i \in \cA$, let $A_i = A \cup \{i\}$.
%         \item Compute $d_i = d(y_{A_i}, y)$ for each $i \in \cA$, and exclude $i$ from $\cA$ such that $d_i > \tau$.
%         \item For each $i \in \cA$ and $j \in \cA_i$, compute $q_{A_i, j}$.
%         \item For each remaining $i \in \cA$, compute
%         \begin{align*}
%             i_t = \argmax_{i \in \cA_k} \sum_{ j \in A_i} q_{A_i,j} b_j,
%         \end{align*}
%         and compute
%         \begin{align*}
%             i_s = \argmax_{i \in \cA_k^{-i_t}} \sum_{ j \in A_i} q_{A_i,j} b_j.
%         \end{align*}
%         \item Compute $p_{i_t} =\sum_{j \in A_{i_s}} q_{A_{i_s},j} b_j -  \sum_{j \in A_{i_t} \setminus\{i_t\}} q_{A_{i_t},j} b_j $
%         \item Update $A \gets A_{i_t}$ and $t \gets t+1$.
%         \item Repeat step $3$ to $6$ until $t = k$.
%         \item Return $A^* = \{i_1,i_2,\ldots, i_k\}$ and charge each $i_t$ the amount of $p_{i_t}$.
%     \end{enumerate}
% \end{definition}

\begin{theorem}
    The mechanism defined in Definition~\ref{def:k-alloc-greedy} has LLM query complexity of $O(nk)$, relevance query complexity of $O(nk)$, and time complexity of $O(nk)$.
\end{theorem}
\begin{proof}
    \sscomment{TODO: polish more.}
    Step $4$ requires at most $O(n)$ queries to the distance oracle and LLM oracle.
    Step $5$ requires $O(n)$ queries to the relevance oracle.
    Then, computing $i_k$ in step $6$ requires $O(n + n)$ computation.
    Step $7$ requires $O(1)$ computation.
    Overall, this requires $O(n)$ queries to the distance oracle, relevance oracle and $O(n)$ computation.
    Since this is repeated for $k$ times, this requires $O(nk)$ queries to the LLM/distance/relevance oracle, and $O(nk)$ computation.
\end{proof}

\SLcomment{Would be good to check whether GSP is actually is a special case of Definiteion 3.21}
    \sscomment{Now that think of it, it is a bit different from GSP since we only care about the set, but not how much prominence each ad is allocated - this is exogenously given in our case now. 
    A bit more precisely, our mechanism does not endogenously compute how much of proportion (prominence) each ad would take in the output, instead we observe how much the ad would be relevant to the given query, \ie the prominence is exogenously given the set of ads to allocate is determined.}


\subsection{Endogenizing $k$.}
So far, we have assumed that the number of allocations $k$ is given in an exogenous manner, and the mechanism only needs to determine a set of ads $A \in \cA_k$ to advertise at once.
Then, one natural question might be how one can determine the parameter $k$.
In terms of social welfare maximizing mechanism, the following ideal mechanism would work albeit its computational complexity.
\begin{theorem}[EPIC mechanism with endogenous $k$]
    Run mechanism defined in Theorem~\ref{thm:k-alloc-epic} for every $k$, and let $A^*_k \in \cA_k$ be the resulting set for $k \in [n]$.
    Then, we pick $k^*$ such that
    \begin{align*}
        k^* = \argmax_{A^*_k :k \in [n]} \sum_{i \in A^*_k} q_{A^*_k, i} b_i.
    \end{align*}
    Then, running $k^*$ allocation EPIC mechanism maximizes the social welfare among every possible multi-allocation (single) mechanism.
\end{theorem}
\begin{proof}
    \sscomment{Simply follows from described mechanism.}
\end{proof}



\begin{definition}[Greedy mechanism with stopping]
    (informal) It runs the same as greedy mechanism in Definition~\ref{def:k-alloc-greedy}, but at each round $t$, after computing $i_t$ and $A_{i_t}$ at step $7$, if the total social welfare at $A_{i_t}$ with $t$ ads is not strictly larger than $A$ with $t-1$ ads, then it breaks and return $A$, and the payment is similarly charged.
\end{definition}

% \begin{example}
%     Give an example that why this is not truthful.
% \end{example}

% \begin{discussion}
%     Discuss that Actually GSP is also a greedy implementation of Second price auction.
% \end{discussion}
If the resulting relevance $q_{A,i}$ for $A \in \cA_k$ and $i \in A$ exhibits arbitrary value, it is impossible to guarantee any reasonable approximation to the EPIC mechanism in terms of the social welfare.
Thus, we impose the following reasonable assumption.
\begin{assumption}[Monotonicity]
    For any $A, B \in \cA_k$ and $i \in A \cap B$, suppose $B \subseteq A$.
    Then, $q_{A.i} \le q_{B,i}$.
\end{assumption}
The assumption essentially implies that whenever more ads are inserted in the final output, each ad suffers loss in terms of the relevance of the ad to the final output, \ie advertiser's utility.
This is fairly plausible since we may want to restrict the total portion of ads in the final output to maintain minimal user experience, and adding more ads necessarily decrease the portion of the existing ads in the output.

\begin{theorem}
    (informal) Under the monotonicity, the greedy mechanism with stopping achieves $O(k)$-approximation for social welfare to the EPIC mechanism with endogenous $k$.
\end{theorem}
\begin{proof}
    \sscomment{Follows from observing the single allocation mechanism and greedy with stopping dominates it.}
\end{proof}




\subsection{Segment-wise Mechanism}
\SLcomment{One way to allocate multiple ads, not as general as this section, might be to do a "RAG-token" style allocation of the ads in the output. The ad that the output is conditioned on could change as the output progresses, e.g. after each paragraph (rather than each token).}
\sscomment{I think we can expand on that at the end of this section - will do that.}

In this mechanism RAG is run for each new discourse segment, where a "segment" here can mean a token, sentence, paragraph, up to the entire output sequence. In other words, depending on the size of the segment, it interpolates between RAG-token and RAG-sequence. Recall that the generative model for the next segment under RAG is:
%
\begin{equation} \label{eq:rag-generative}
p(y|x) = \sum_{i \in \cA} p_{\eta}(z_i | x; \b) p_{\theta}(y | x, z_i)
\end{equation}
%
We want to run an auction to assign each bidder $i$ to generate the next segment with probability $p_{\eta}(z_i | x; \b)$, and price so that it is truthful. Here is such an auction.
%
\begin{itemize}
    \item Define the disjoint intervals $W_i = \left[ 
    \sum_{j < i} p_{\eta}(z_i | x; \b), \sum_{j \leq i} p_{\eta}(z_i | x; \b)
    \right]$ for $i \in \cA$ \sscomment{Is this $p(z_j | x;\b)$?} \SLcomment{Correct, the width of this interval is $p(z_i | x;\b)$, so advertiser $i$ wins with that probability as desired.}
    \item Draw $t \sim \mathrm{Uniform}(0, 1)$
    \item Let $k$ be the ad such that $t \in W_k$.
    \item Output $y \sim p_{\theta}(\cdot | x, z_k)$.
    \item Charge $k$ the smallest bid $\bar{b}_k$ such that $t \in W_k$.
    \sscomment{This looks similar to randomized mechanism akin to FAIR mechanism we have (at least for allocation) for each segment (If it were to be the simple aggregation function below). But the payment rule seems to be different from FAIR. What am I missing here?} \SLcomment{Let's talk in person about how we each came up with the payment rules for FAIR and the segment-wise mechanism here. You're right that they're closely related, since FAIR finds a probabilistic allocation that can align with the RAG selection probabilities.}
    \sscomment{Essentially this looks similar to segment-wise mechanism leveraging single-allocation mechanism that we previously discussed, but using randomized allocation, please fix me if I'm wrong.} \SLcomment{The important point is that the randomized allocation is the one dictated by RAG (after a suitable aggregation function via bids).}
\end{itemize}
\sscomment{In generating the next segment $y$, does this not condition on the previous segments?}
%
It's easy to see that the auction selects an ad and outputs $y$ according to the generative model~\eqref{eq:rag-generative}. For each realization of $t$, the auction is truthful, by the same arguments as for a second-price auction. Therefore, the auction is truthful.


To evaluate the payment $\bar{b}_k$ we need to specify the aggregation function for probabilities. Consider the simple form:
$$
p_{\eta}(z_i | x; \b) = \frac{b_i p_{\eta}(z_i | x)}{\sum_j b_j p_{\eta}(z_i | x)}
$$
where $p_{\eta}(z_i | x)$ is the default selection probability for ad $i$, which would occur if all bids were equal. For simplicity we just write $p_i$ for $p_{\eta}(z_i | x)$. The explicit formula for $\bar{b}_k$ under this aggregation function is as follows:
%
\begin{itemize}
    \item Case 1: $\sum_{j < k} \frac{p_j b_j}{\sum_{\ell \neq k} p_\ell b_\ell} \geq t$ \\
    \[
    \bar{b}_k = \frac{\sum_{j < k} p_j b_j - t \sum_{\ell \neq k} p_\ell b_\ell}{t p_k}
    \]
    %
    \item Case 2: $\sum_{j < k} \frac{p_j b_j}{\sum_{\ell \neq k} p_\ell b_\ell} \leq t$ \\
    \[
    \bar{b}_k = \frac{\sum_{j < k} p_j b_j - t \sum_{\ell \neq k} p_\ell b_\ell}{(t-1) p_k}
    \]
    
\end{itemize}

\SLcomment{It would be interesting to characterize what objective function the RAG generative model~\eqref{eq:rag-generative} optimizes. This again depends on the aggregation function.}
\sscomment{To define objective function, we should define what the advertiser's utility is. We may assume that advertiser's utility is additive over each segment. But it's still not clear what such allocation maximizes, mainly because if we tweak a certain segment in the middle, this would change the entire next segments (assuming that future segment is generated w.r.t. previous ones), and we don't know the relationship between two corresponding output.} \SLcomment{The advertiser utility is just the value per click (or the bid) minus the payment per click, all multiplied by CTR. The objective function will be some function of the value (or bids) only, not the payments.}

\SLcomment{We could also work out the payment rule for the log-linear aggregation function from Renato's paper.}

\SLcomment{We can introduce a "reserve" price $r$ by adding another bidder that bids $r$, and if it wins, no ad is introduced into the prompt. What is the revenue-optimal reserve price in that case? We could work through a Myerson-style analysis. Not sure how insightful this would be though.}

The idea is that if an ad "wins" for a segment, then it is introduced into the prompt for generating that segment, and the ad may then get mentioned in the segment. For example, a link to the advertiser's website would be included. So it seems particularly important here that the payment is charged \emph{per click}, because there is a chance the LLM will not end up mentioning the ad. The probability of click could be related to the cosine similarity of the ad embedding with the prompt embedding, as in the experimental colab. This is different from other ad auctions like Search or Display, where if an ad wins it is guaranteed to be shown, but of course there's no guarantee of a click. In that setup, it's possible to charge "per impression".

\SLcomment{We can make the segment-wise auction similar to GSP as follows. Say we're generating paragraphs one at a time. If the winning advertiser (say $k$) is shown in the first paragraph, remove it from the set of advertisers. Next run the segment auction for the next paragraph with the remaining bidders. This will have the property that the bidder with the highest bid is most likely to be shown first, etc. (similar to GSP). We could also introduce a "position discount factor" such that the CTR of an ad depends on its relevance to the query (according to e.g. embedding cosine similarity) multiplied by a paragraph-dependent factor, where lower paragraphs have smaller factors. This is just like position factors in GSP.}



% Then, similar to Section~\ref{subsec:desiderata}, we are interested in DSIC, IR, and welfare maximizing mechanism, where welfares are analogously defined as follows.

% \subsection{Further Discussions}

% \paragraph{Valuation model}

% If $A$ were to be $\{i\}$, then we can essentially use $q_i \cdot v_i $ of Definition~\ref{def:rel-value}.

% \begin{definition}[Valuation]
%     Given a query $x$ and the corresponding relevance $q_A = r(a_A | x)$, the advertiser $i$'s true valuation of advertising $a_i$ is $\tv_i = q_i \cdot v_i$. We also write $\tb_i = q_ib_i$ instead of $\tv_i$ when we deal with the bid instead of the valuation.
% \end{definition}



